Learnable Permutation for Structured Sparsity on Transformer Models

Structured sparsity has emerged as a popular model pruning technique, widely adopted in various architectures, including CNNs, Transformer models, and especially large language models (LLMs) in recent years. A promising direction to further improve post-pruning performance is weight permutation, which reorders model weights into patterns more amenable to pruning. However, the exponential growth of the permutation search space with the scale of Transformer architectures forces most methods to rely on greedy or heuristic algorithms, limiting the effectiveness of reordering. In this work, we propose a novel end-to-end learnable permutation framework. Our method introduces a learnable permutation cost matrix to quantify the cost of swapping any two input channels of a given weight matrix, a differentiable bipartite matching solver to obtain the optimal binary permutation matrix given a cost matrix, and a sparsity optimization loss function to directly optimize the permutation operator. We extensively validate our approach on vision and language Transformers, demonstrating that our method achieves state-of-the-art permutation results for structured sparsity.

==> sections/abstract.tex <==
\begin{abstract}


Structured sparsity has emerged as a popular model pruning technique, widely adopted in various architectures, including CNNs, Transformer models, and especially large language models (LLMs) in recent years. A promising direction to further improve post-pruning performance is weight permutation, which reorders model weights into patterns more amenable to pruning. However, due to the vast permutation search space, most existing methods rely on greedy or heuristic algorithms, limiting the potential benefits of reordering.

In this work, we propose a novel \textbf{end-to-end learnable} permutation framework. Our method introduces a learnable permutation cost matrix {\textcolor{red}{to}}, a differentiable bipartite matching solver {\textcolor{red}{to}}, and a sparsity-aware loss function to directly optimize the permutation operator.
We extensively validate our approach on both vision transformers and LLMs, demonstrating that our method achieves state-of-the-art permutation results for structured sparsity.


\end{abstract}

==> sections/abstract_v2.tex <==
\begin{abstract}


Structured sparsity has emerged as a popular model pruning technique, widely adopted in various architectures, including CNNs, Transformer models, and especially large language models (LLMs) in recent years. A promising direction to further improve post-pruning performance is weight permutation, which reorders model weights into patterns more amenable to pruning. However, the exponential growth of the permutation search space with the scale of Transformer architectures forces most methods to rely on greedy or heuristic algorithms, limiting the effectiveness of reordering.


In this work, we propose a novel \textbf{end-to-end learnable} permutation framework. Our method introduces a learnable permutation cost matrix to quantify the cost of swapping any two input channels
of a given weight matrix, a differentiable bipartite matching solver to obtain the optimal binary permutation matrix given a cost matrix, and a sparsity optimization loss function to directly optimize the permutation operator.
We extensively validate our approach on vision and language Transformers, demonstrating that our method achieves state-of-the-art permutation results for structured sparsity.


\end{abstract}

==> sections/experiments.tex <==



\section{Experiments}

% ------------------------------------------------------------------
% Language results (7B LLM, 2:4 sparsity, evaluation on reasoning suites)
% ------------------------------------------------------------------


\begin{table}[]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|c|c|cc}
\toprule
\textbf{Model} & \textbf{Sparsity} & \textbf{Method} & \textbf{Top-1 (\%)} & \textbf{Top-5 (\%)} \\ \midrule
\multirow{9}{*}{ViT-Base/16} & 0\% & Dense & 79.1 & 94.1 \\ \cmidrule{2-5} 
 & \multirow{4}{*}{2:4} & CP & 66.2 & 86.4 \\
 &  & Wanda & 65.8 & 86.4 \\
 &  & RIA & 66.6 & 86.6 \\
 &  & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}\textbf{67.9} & \cellcolor{yellow!15}\textbf{87.9} \\ \cmidrule{2-5} 
 & \multirow{4}{*}{4:8} & CP & 66.8 & 88.2 \\
 &  & Wanda & 66.4 & 86.6 \\
 &  & RIA & 71.4 & 89.9 \\
 &  & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}\textbf{71.8} & \cellcolor{yellow!15}\textbf{90.2} \\ \midrule
\multirow{9}{*}{ViT-Large/14} & 0\% & Dense & 85.2 & 97.9 \\ \cmidrule{2-5} 
 & \multirow{4}{*}{2:4} & CP & 79.5 & 94.7 \\
 &  & Wanda & 79.2 & 95.2 \\
 &  & RIA & 79.6 & 95.1 \\
 &  & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}\textbf{80.7} & \cellcolor{yellow!15}\textbf{95.8} \\ \cmidrule{2-5} 
 & \multirow{4}{*}{4:8} & CP & 82.0 & 96.4 \\
 &  & Wanda & 82.0 & 96.4 \\
 &  & RIA & 82.3 & 96.4 \\
 &  & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}\textbf{82.7} & \cellcolor{yellow!15}\textbf{96.5} \\ \bottomrule
\end{tabular}}
\caption{Accuracy on ImageNet after pruning ViT-Base/16 and ViT-Large/14 to the 2:4 and 4:8 structured pattern (50\,\% non-zero weights).}
\label{tab:vit_results}
\end{table}


\subsection{Experimental Setup}

\subsubsection{Models.} We evaluate our learnable permutation framework for structured sparsity on several popular Transformer backbones that span both vision and language domains. For vision domain, we select commonly used \texttt{ViT-Base/16} and \texttt{ViT-Large/14}~\cite{dosovitskiy2020image} for experiments. 
For language domain, we employ \texttt{LLaMA-3.2-1B} and \texttt{LLaMA-2-7B}~\cite{touvron2023LLaMA} to represent the common small and large language models. For multimodal domain, we chose \texttt{Qwen2.5-VL-3B}~\cite{bai2025qwen2} as the object of study.


\subsubsection{Datasets.} For the vision tasks, we use the canonical \texttt{ImageNet-1K} dataset~\cite{deng2009imagenet}, which consists of 1.28M training images and 50K validation images. All models are trained with the official train/validation split with standard input resolution of $224^2$. 
For the language modeling tasks, permutations are learned on a training set of \texttt{C4} dataset~\cite{raffel2020exploring}, which comprises approximately 783MB of cleaned English text.


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|c|ccccccc|c}
\toprule
\textbf{Model} & \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Wikitext2} & \textbf{Arc-Easy} & \textbf{Arc-Challenge} & \textbf{BoolQ} & \textbf{HellaSwag} & \textbf{OpenBookQA} & \textbf{WinoGrande} & \textbf{MMLU} & \textbf{Average} \\ \midrule
\multirow{8}{*}{\shortstack[c]{LLaMA‑3.2‑1B\\(2:4)}} & Dense & 9.06 & 65.36 & 31.40 & 63.82 & 47.73 & 26.60 & 60.69 & 31.19 & 46.68 \\ \cmidrule{2-11} 
 & Magnitude & 4808.42 & 27.95 & 19.45 & 38.50 & 26.13 & 11.80 & 51.78 & 23.80 & 28.49 \\
 & SparseGPT & 32.20 & 45.29 & 20.65 & 62.11 & 31.99 & 15.20 & 54.54 & 24.68 & 36.35 \\
 & Wanda & 75.76 & 37.16 & 18.17 & 62.05 & 28.57 & 12.00 & 50.20 & 24.45 & 33.23 \\
 & PrunerZero & 141.40 & 36.70 & 19.28 & 57.43 & 27.72 & 13.40 & 50.12 & 25.72 & 32.91 \\
 & CP & 68.17 & 38.35 & 18.14 & 62.08 & 28.56 & 12.40 & 53.31 & 23.82 & 33.81 \\
 & RIA & 72.56 & 38.12 & 20.33 & 61.34 & 27.12 & 12.80 & 52.76 & 24.31 & 33.83 \\
 & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}45.32 & \cellcolor{yellow!15}42.27 & \cellcolor{yellow!15}21.08 & \cellcolor{yellow!15}62.12 & \cellcolor{yellow!15}29.12 & \cellcolor{yellow!15}15.60 & \cellcolor{yellow!15}54.82 & \cellcolor{yellow!15}26.27 & \cellcolor{yellow!15}35.90 \\ \midrule
\multirow{8}{*}{\shortstack[c]{LLaMA‑2‑7B\\(2:4)}} & Dense & 5.12 & 76.30 & 43.43 & 77.68 & 57.14 & 31.40 & 69.06 & 45.84 & 57.26 \\ \cmidrule{2-11} 
 & Magnitude & 52.00 & 61.87 & 30.20 & 59.79 & 45.42 & 21.80 & 60.93 & 26.87 & 43.84 \\
 & SparseGPT & 10.30 & 64.10 & 32.51 & 71.25 & 43.35 & 25.00 & 67.25 & 28.56 & 47.43 \\
 & Wanda & 11.38 & 62.75 & 30.38 & 67.65 & 41.18 & 23.60 & 62.59 & 27.82 & 45.14 \\
 & PrunerZero & 12.91 & 61.20 & 27.47 & 66.15 & 39.43 & 24.40 & 61.01 & 27.41 & 43.87 \\
 & CP & 10.68 & 63.32 & 30.96 & 66.92 & 41.32 & 23.80 & 63.56 & 26.51 & 45.20 \\
 & RIA & 10.52 & 63.67 & 31.82 & 67.13 & 42.03 & 23.00 & 64.13 & 27.56 & 45.62 \\
 & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}10.17 & \cellcolor{yellow!15}64.22 & \cellcolor{yellow!15}31.96 & \cellcolor{yellow!15}68.17 & \cellcolor{yellow!15}43.31 & \cellcolor{yellow!15}23.60 & \cellcolor{yellow!15}63.79 & \cellcolor{yellow!15}28.13 & \cellcolor{yellow!15}46.17 \\ \bottomrule
\end{tabular}}
\caption{Evaluation of the LLaMA2-7B language model after 2:4 structured pruning. Average (\%) is the accuracy retention relative to the dense baseline.}
\label{tab:nlp_results}
\end{table*}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|c|ccccccc|c}
\toprule
\textbf{Model} & \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Wikitext2} & \textbf{Arc-Easy} & \textbf{Arc-Challenge} & \textbf{BoolQ} & \textbf{HellaSwag} & \textbf{OpenBookQA} & \textbf{WinoGrande} & \textbf{MMLU} & \textbf{Average} \\ \midrule
\multirow{8}{*}{\shortstack[c]{LLaMA‑2‑7B\\(4:8)}}
 & Dense & 5.12 & 76.30 & 43.43 & 77.68 & 57.14 & 31.40 & 69.06 & 45.84 & 57.96 \\ \cmidrule{2-11}
 & Magnitude & 16.23 & 64.69 & 35.92 & 62.63 & 50.08 & 26.00 & 62.27 & 28.07 & 47.09 \\
 & SparseGPT & 7.84 & 69.61 & 36.77 & 72.11 & 48.27 & 27.40 & 68.35 & 32.81 & 50.76 \\
 & Wanda & 8.07 & 67.26 & 34.30 & 73.91 & 46.95 & 26.20 & 66.81 & 26.11 & 48.76 \\
 & PrunerZero & 8.52 & 65.70 & 33.36 & 69.27 & 45.58 & 23.20 & 66.30 & 28.81 & 47.46 \\
 & Perm & 8.11 & 66.92 & 34.51 & 72.88 & 46.18 & 26.17 & 66.64 & 26.13 & 48.49 \\
 & RIA & 7.92 & 67.85 & 33.92 & 72.26 & 47.12 & 27.32 & 66.89 & 26.82 & 48.88 \\
 & \cellcolor{yellow!15}Ours & \cellcolor{yellow!15}7.61 & \cellcolor{yellow!15}68.51 & \cellcolor{yellow!15}35.02 & \cellcolor{yellow!15}73.88 & \cellcolor{yellow!15}47.63 & \cellcolor{yellow!15}28.15 & \cellcolor{yellow!15}66.73 & \cellcolor{yellow!15}28.67 & \cellcolor{yellow!15}49.80 \\
\bottomrule
\end{tabular}
}
\caption{Performance of different methods on LLaMA2-7B model after 2:4 structured pruning.}
\label{tab:your_label_here}
\end{table*}


\subsubsection{Baselines.} Our method is compared with a variety of classic and state-of-the-art pruning baselines, including Magnitude~\cite{han2015learning}, Wanda \cite{sun2023wanda}, SparseGPT \cite{frantar2023sparsegpt}, PrunerZero~\cite{dong2024pruner}, CP \cite{pool2021channel}, RIA \cite{zhangplug}, and E-Sparse \cite{li2023sparse}.


\subsubsection{Evaluations.} For vision model evaluations, we use the canonical \texttt{ImageNet-1K} validation dataset with top-1/5 accuracy as the primary metric. 
For language model evaluations, we adopt perplexity as an evaluation metric to assess language comprehension ability, measured on the \texttt{WikiText2} test set~\cite{merity2016pointer}. To assess the effect of compression on a wide range of downstream tasks, we report zero-shot accuracy on \texttt{ARC}~\cite{allenai:arc}, \texttt{BoolQ}~\cite{clark2019boolq}, \texttt{HellaSwag}~\cite{zellers2019hellaswag}, \texttt{OpenBookQA}~\cite{OpenBookQA2018}, and \texttt{WinoGrande}~\cite{sakaguchi2021winogrande}, along with five-shot accuracy on the \texttt{MMLU} benchmark\cite{hendrycks2020measuring}.
For multimodal evaluations, we report zero-shot \texttt{MMMU}~\cite{yue2024mmmu}, \texttt{MMStar}~\cite{chen2024we}, and \texttt{TextVQA}~\cite{singh2019towards} accuracy.

\subsubsection{Implementation Details.}
Vision models are trained for 20 epochs on 2 AMD MI250 GPUs with AdamW (weight decay $0.01$, base learning rate $0.1$) under a cosine decay schedule and no warm-up.  Language models are trained for 20 update epochs with AdamW ($\text{lr}=10^{-4}$); the default permutation group number $G$ is 8; all runs use native AMP with FP16 precision, gradient accumulation set to one, and a small Smooth-L1 distillation term weighted $10^{-5}$.  Random seeds are fixed to 42.

\subsection{Performance Results}

\subsubsection{Results on Vision Transformers.}
On the vision side, we apply structured pruning to \texttt{ViT-Base/16} and \texttt{ViT-Large/14} under the 2:4 and 4:8 sparsity patterns, retaining 50\% of the weights. Across all settings, our method consistently achieves the highest top-1 and top-5 accuracy among the compared approaches. For \texttt{ViT-Base/16}, our method obtains 67.9\% / 87.9\% (top-1 / top-5) accuracy at 2:4 sparsity, outperforming the strongest baseline (RIA) by 1.3\%age points. At 4:8 sparsity, it further improves to 71.8\% / 90.2\%, slightly ahead of RIA by 0.4 and 0.3 points. Similar trends are observed on \texttt{ViT-Large/14}, where our method reaches 80.7\% / 95.8\% at 2:4 sparsity and 82.7\% / 96.5\% at 4:8 sparsity, both surpassing prior methods. These results highlight the effectiveness of our approach in preserving accuracy for Vision Transformers.

\begin{table}[t]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
  \begin{tabular}{@{}c|l|c|c|c|c@{}}
    \toprule
    Sparsity & Method     & MMMU & MMStar & TextVQA & Average \\
    \midrule
    0\%  & Dense       & 53.1 & 55.8 & 79.3   & 62.7    \\
    \midrule
    \multirow{4}{*}{2:4}
         & Magnitude   & 34.1 & 48.7   & 76.5 & 53.1   \\
         & Wanda       & 37.2 & 51.2   & 77.2 & 55.2   \\
         & RIA         & 37.3 & 51.4   & 77.1 & 55.3   \\
         & \cellcolor{yellow!15}Ours
         & \cellcolor{yellow!15}\textbf{38.1}
         & \cellcolor{yellow!15}\textbf{51.9}
         & \cellcolor{yellow!15}\textbf{77.8} 
         & \cellcolor{yellow!15}\textbf{55.9} \\
    \bottomrule
  \end{tabular}
  \caption{Qwen2.5-VL-3B performance under different pruning methods and sparsity levels.}
  \label{tab:mmmu_pruning}
\end{table}

\subsubsection{Results on Language Transformers.}
On the language side, we evaluate pruning performance on both \texttt{LLaMA-3.2-1B} and \texttt{LLaMA-2-7B} models across a range of context modeling and commonsense benchmarks. Our method—using Wanda pruning followed by a learned channel permutation—consistently improves downstream performance over baseline methods without requiring weight updates. On \texttt{LLaMA-3.2-1B}, our approach improves the average accuracy to 35.90\%, outperforming Wanda (33.23\%), CP (33.81\%), and RIA (33.83\%) by 2.1 to 2.7 points. Similar trends are observed on \texttt{LLaMA-2-7B}, where our method reaches 46.17\% average accuracy, compared to 45.14\% (Wanda), 45.20\% (CP), and 45.62\% (RIA). Notably, our method improves performance on challenging tasks such as \texttt{ARC-Challenge} (e.g., +3.79 points over Wanda for LLaMA-3.2-1B) and maintains strong results on \texttt{BoolQ} and \texttt{WinoGrande}. While methods like SparseGPT achieve higher accuracy due to weight updates, our approach operates in the same constrained setting as Wanda, offering a fair and efficient comparison. Moreover, on \texttt{WikiText2}, our method yields significantly better perplexity than SparseGPT and PrunerZero, demonstrating its ability to preserve language modeling quality under structured sparsity.

\subsubsection{Results on Multimodal Transformers.}
As shown in Table~\ref{tab:mmmu_pruning}, our method achieves the highest performance among all evaluated 2:4 structured pruning approaches on the \texttt{MMMU} benchmark using the \texttt{Qwen2.5-VL-3B} model. While traditional methods such as Magnitude pruning and recent techniques like Wanda and RIA yield scores of 34.1, 37.2, and 37.3 respectively, our approach outperforms them with a score of 37.9, demonstrating its effectiveness in preserving critical information under structured sparsity constraints. 


For Transformer-based models of various types, the learnable permutation consistently lifts performance beyond magnitude-only or rule-based permutation strategies, and does so while preserving the full latency advantage of $2{:}4$ sparsity.  The effect is especially pronounced on benchmarks that rely on multi-step reasoning, suggesting that permutation learning helps concentrate semantically aligned features into the survivable positions of each weight block.

% ------------------------------------------------------------------
% Vision results (ImageNet, ViT-Base/16)
% ------------------------------------------------------------------

%\begin{table}[t]
%\centering
%\caption{Top-1 accuracy on ImageNet after pruning ViT-Base/16 to the $2{:}4$ structured pattern
%(50\,\% non-zero weights).}
%\label{tab:vit_results}
%\begin{tabular}{lcc}
%\toprule
%\textbf{Method} & \textbf{Sparsity (\%)} & \textbf{Top-1 (\%)} \\
%\midrule
%Dense baseline & 0 & 82.1 \\
%Channel Pruning (CP) & 50 & 66.5 \\
%Recurrent Importance Allocation (RIA) & 50 & 66.8 \\
%\textbf{Ours: Wanda + learn2perm} & 50 & \textbf{67.4} \\
%\bottomrule
%\end{tabular}
%\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



% Please add the following required packages to your document preamble:
% 


\begin{table}[t]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
  \begin{tabular}{@{}c|c|c c c|c@{}}
    \toprule
    Epochs & Wikitext2 & Arc‑Easy & Arc‑Chall. & MMLU & Average \\
    \midrule
      0  & 11.38 & 62.75 & 30.38 & 27.82 & 40.32 \\
      1  & 10.56 & 62.89 & 30.92 & 27.61 & 40.47 \\
      2  & 10.31 & 63.15 & 31.02 & 27.96 & 40.71 \\
      5  & 10.27 & 64.10 & 31.92 & 28.05 & 41.36 \\
     10  & 10.21 & \textbf{64.23} & 31.88 & 28.12 & 41.41 \\
     \cellcolor{yellow!15}20  & \cellcolor{yellow!15}10.17 & \cellcolor{yellow!15}64.22 & \cellcolor{yellow!15}\textbf{31.96} & \cellcolor{yellow!15}\textbf{28.13} & \cellcolor{yellow!15}\textbf{41.44} \\
    \bottomrule
  \end{tabular}
  \caption{Performance over different training epochs.}
  \label{tab:epoch_results}
\end{table}

\begin{table*}[t]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
  \begin{tabular}{@{}c|c|c|c|c c c c c c c|c@{}}
    \toprule
    Group & Trainable & Time & Wikitext2 & Arc‑Easy & Arc‑Chall. & BoolQ & HellaSwag & OpenBookQA & WinoGrande & MMLU & Average \\
    \midrule
      1  & 51.31\% & $\sim$4h  & 10.11 & 64.89 & 32.04 & 68.02 & 43.56 & 23.80 & 63.92 & 28.07 & 46.33 \\
      2  & 34.92\%   & $\sim$4h  & 10.12 & 64.35 & 31.84 & 68.21 & 43.82 & 23.60 & 64.02 & 28.25 & 46.30 \\
  \rowcolor{yellow!15}
      4  & 20.85\%  & $\sim$4h  & 10.17 & 64.22 & 31.96 & 68.17 & 43.31 & 23.60 & 63.79 & 28.13 & 46.17 \\
      8  & 11.64\%   & $\sim$6h  & 10.25 & 64.15 & 31.82 & 68.21 & 43.15 & 23.60 & 63.82 & 28.15 & 46.13 \\
     16  & 6.18\%    & $\sim$9h  & 10.63 & 63.59 & 31.15 & 67.92 & 42.89 & 23.00 & 63.72 & 27.67 & 45.71 \\
    \bottomrule
  \end{tabular}
  \caption{Performance of \textsc{LLaMA‑2‑7B} with different permutation group numbers, including training cost and parameter ratio.}
  \label{tab:group_results}
\end{table*}




\begin{table*}[t]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{@{}l|l|c|c c c c c c c|c@{}}
    \toprule
    Model & Pruning Baseline & Wikitext2 & Arc‑Easy & Arc‑Chall. & BoolQ & HellaSwag & OpenBookQA & WinoGrande & MMLU & Average \\
    \midrule
    \multirow{4}{*}{LLaMA‑2‑7B}
      & Magnitude+ours    & 45.82 & 62.89 & 30.90 & 61.68 & \textbf{45.47} & 22.20 & 62.12 & 27.12 & 44.63 \\
      & Wanda+ours        & 10.17 & 64.22 & 31.96 & 68.17 & 43.31 & 23.60 & 63.79 & 28.13 & 46.17 \\
      & RIA+ours          & 10.02 & 63.88 & 32.53 & \textbf{68.83} & 42.59 & 24.00 & 64.32 & 29.02 & 46.45 \\
      & AdmmPruner+ours   &  \textbf{9.56} & \textbf{69.02} & 32.68 & 63.41 & 45.12 & \textbf{26.00} & \textbf{65.96} & \textbf{29.62} & \textbf{47.40} \\
    \bottomrule
  \end{tabular}}
  \caption{Performance on different pruning baselines for \textsc{LLaMA‑2‑7B}.}
  \label{tab:more_baselines}
\end{table*}

\begin{table}[t]
  \centering
  
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l|c|c|c|c|c|c@{}}
      \toprule
      Loss & Wikitext2 & Arc‑Easy & Arc‑Chall. & WinoGrande & MMLU & Average \\
      \midrule
      Pres.\_mag\_sum           & 568.72 & 30.25 & 19.56 & 51.69 & 23.96 & 31.37 \\
      Pres.\_wanda\_metric\_sum & 62.14  & 39.43 & 18.83 & 51.88 & 25.71 & 33.96 \\
      Pres.\_ria\_metric\_sum   & 65.43  & 38.91 & 19.89 & 52.36 & 25.19 & 34.09 \\
      CE loss                   & 46.15  & 42.01 & 20.53 & 53.97 & 26.12 & 35.66 \\
      Distill loss              & 52.58  & 40.51 & 20.12 & 52.83 & 25.97 & 34.86 \\
      \cellcolor{yellow!15}CE+Distill loss           & \cellcolor{yellow!15}45.32  & \cellcolor{yellow!15}42.27 & \cellcolor{yellow!15}21.08 & \cellcolor{yellow!15}54.82 & \cellcolor{yellow!15}26.27 & \cellcolor{yellow!15}36.11 \\
      \bottomrule
    \end{tabular}}
    \caption{Performance of different loss configurations across benchmarks.}
  \label{tab:loss}
\end{table}


\subsection{Training Convergence and Efficiency}
To assess training convergence, we track performance from the very start of training (epoch 1) to 20 epochs, as shown in Table~\ref{tab:epoch_results}. The initial point is weak (average 33.23, \texttt{Wikitext2} perplexity 75.76), but after just one epoch the average jumps to 40.47 and perplexity drops to 10.56, an approximately 86\% reduction, showing the permutator is extremely fast to optimize. Longer training continues to help but with clear saturation: 40.71 at 2 epochs, 41.36 at 5, 41.41 at 10, and 41.44 at 20. Across tasks, \texttt{Arc‑Easy} improves from 37.16 to 64.22, \texttt{Arc‑Challenge}. from 18.17 to 31.96, and \texttt{MMLU} from 24.45 to 28.13, with most gains already achieved in the first epoch, which takes 3 to 4 hours approximately.
Overall, the results highlight the rapid convergence and training efficiency of our method: nearly all attainable accuracy is achieved within just five epochs—only 0.08 below the performance at 20 epochs—making it an ideal default. Moreover, each epoch is computationally lightweight, further underscoring the method’s suitability for efficient training.


\subsection{Ablation Study}

\subsubsection{Impact of Permutation Group Number.}
We study how the number of permutation groups $G$ (i.e., how finely we partition a weight matrix before learning permutations) influences both effectiveness and efficiency. A smaller $G$ (larger groups) allows the permutator to explore more global reorderings, which should yield better permutation masks. A larger $G$ (smaller groups) shrinks the learnable permutator, reducing parameters and training time, but also constrains the search space.
As shown in Table~\ref{tab:group_num}, We evaluate $G\in\{1,2,4,8,16\}$ on LLaMA‑2‑7B.
The average score decreases only slightly from 46.33 (G=1) to 46.30, 46.17, 46.13, 45.71 as group number increases. Wikitext2 perplexity rises from 10.11 to 10.63. The largest task drop is on Arc‑Easy (64.89 to 63.59). Between G=4 and 8 the average differs by just 0.04, showing diminishing returns once moderate group sizes are allowed.
The permutator's parameter count and training time shrink roughly in proportion to the number of groups. Moving from G=1 to 4 cuts the cost by about 16$\times$ for only a 0.16 drop in the average score, while G=2 is almost identical to G=1 (-0.03). We therefore adopt G=4 as the default in the rest of the paper.

On the other hand, trainable parameters are 51.31\% for group 1, 34.92\% for group 2, 20.85\% for group 4, 11.64\% for group 8, and 6.18\% for group 16, while wall clock time is about 4 hours for groups 1 to 4, about 6 hours for group 8, and about 9 hours for group 16. Relative to group 1, group 4 reduces trainable parameters by about 59\% with essentially unchanged average score from 46.33 to 46.17 and no extra time; moving to groups 8 and 16 cuts parameters further but changes the average score by only 0.04 and 0.46 while increasing time by about 50\% and 125\%. We therefore adopt group 4 by default.



\subsubsection{Performance over different pruning baselines.}
To assess the generality of our approach, we incorporate the learnable permutator into four distinct pruning baselines: Magnitude, Wanda, RIA, and AdmmPruner. As shown in Table~\ref{tab:more_baselines}, our method consistently improves performance across all cases. Specifically, the average score of Magnitude increases from 43.84 to 44.63, Wanda from 45.14 to 46.17, and RIA from 45.62 to 46.45. Wikitext2 perplexity is reduced in every case—for instance, from 52.00 to 45.82 for Magnitude, from 11.38 to 10.17 for Wanda, and from 10.52 to 10.02 for RIA. On MMLU, the scores improve from 26.87, 27.82, and 27.56 to 27.12, 28.13, and 29.02, respectively. Moreover, our permutator is compatible with post-pruning weight updates: when combined with AdmmPruner, it achieves the highest overall average (47.40), the best MMLU score (29.62), and the lowest Wikitext2 perplexity (9.56). These results demonstrate that the proposed permutator is broadly applicable and complementary to existing pruning strategies and post-pruning optimization techniques.


\subsubsection{Impact of different training objectives.}
To understand how to train the permutator, we compare indirect objectives that try to preserve weight statistics with end to end objectives that optimize the model outputs directly. Table \ref{tab:loss} shows that the indirect objectives are clearly weaker: preserved magnitude reaches an average of 31.37 with a very high Wikitext2 perplexity of 568.72, while the Wanda and RIA metric sums reach 33.96 and 34.09. In contrast, end to end signals are consistently better. Cross entropy on the final outputs attains an average of 35.66 with a much lower perplexity of 46.15, and the layer wise distillation loss reaches 34.86. Using both together yields the best overall result: an average of 36.11, the strongest scores on Arc Easy (42.27), Arc Challenging (21.08), WinoGrande (54.82), and MMLU (26.27), and a competitive perplexity of 45.32. These observations indicate that indirect weight based heuristics are insufficient for steering the permutation, while both cross entropy and layer wise distillation effectively guide learning, and their combination provides the most reliable gains.





==> sections/experiments_v2.tex <==



\section{Experiments}

% ------------------------------------------------------------------
% Language results (7B LLM, 2:4 sparsity, evaluation on reasoning suites)
% ------------------------------------------------------------------


\begin{table}[]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{c|c|c|cc}
\toprule
\textbf{Model} & \textbf{Sparsity} & \textbf{Method} & \textbf{Top-1 (\%)} & \textbf{Top-5 (\%)} \\ \midrule
\multirow{9}{*}{ViT-Base/16} & 0\% & Dense & 79.1 & 94.1 \\ \cmidrule{2-5} 
 & \multirow{4}{*}{2:4} & CP & 66.2 & 86.4 \\
 &  & Wanda & 65.8 & 86.4 \\
 &  & RIA & 66.6 & 86.6 \\
 &  & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}\textbf{67.9} & \cellcolor{gray!20}\textbf{87.9} \\ \cmidrule{2-5} 
 & \multirow{4}{*}{4:8} & CP & 66.8 & 88.2 \\
 &  & Wanda & 66.4 & 86.6 \\
 &  & RIA & 71.4 & 89.9 \\
 &  & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}\textbf{71.8} & \cellcolor{gray!20}\textbf{90.2} \\ \midrule
\multirow{9}{*}{ViT-Large/14} & 0\% & Dense & 85.2 & 97.9 \\ \cmidrule{2-5} 
 & \multirow{4}{*}{2:4} & CP & 79.5 & 94.7 \\
 &  & Wanda & 79.2 & 95.2 \\
 &  & RIA & 79.6 & 95.1 \\
 &  & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}\textbf{80.7} & \cellcolor{gray!20}\textbf{95.8} \\ \cmidrule{2-5} 
 & \multirow{4}{*}{4:8} & CP & 82.0 & 96.4 \\
 &  & Wanda & 82.0 & 96.4 \\
 &  & RIA & 82.3 & 96.4 \\
 &  & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}\textbf{82.7} & \cellcolor{gray!20}\textbf{96.5} \\ \bottomrule
\end{tabular}}
\caption{Performance of different approaches on ImageNet after pruning ViT-Base/16 and  ViT-Large/14 to the 2:4 and 4:8 structured pattern (50\,\% non-zero weights).}
\label{tab:vit_results}
\vspace{-4mm}
\end{table}


\subsection{Experimental Setup}

\subsubsection{Models.} We evaluate our learnable permutation framework for structured sparsity on several popular Transformer backbones that span both vision and language domains. For vision domain, we select commonly used \texttt{ViT-Base/16} and \texttt{ViT-Large/14}~\cite{dosovitskiy2020image} for experiments. 
For language domain, we employ \texttt{LLaMA-3.2-1B}~\cite{dubey2024llama} and \texttt{LLaMA-2-7B}~\cite{touvron2023llama} to represent the common small and large language models. For multimodal domain, we chose \texttt{Qwen2.5-VL-3B}~\cite{bai2025qwen2} as the object of study.


\subsubsection{Datasets.} For the vision transformers, we use the canonical \texttt{ImageNet-1K} dataset~\cite{deng2009imagenet}, which consists of 1.28M training images and 50K validation images. All models are trained with the official train/validation split with standard input resolution of $224 \times 224$. 
For the language models, permutations are learned on the training set of \texttt{C4} dataset~\cite{raffel2020exploring} and Alpaca-en dataset~\cite{alpaca}, which comprises approximately 806MB of cleaned English text. For the vision-language models, permutations are learned on the training set of  Alpaca-en dataset~\cite{alpaca} and LLaVA-Instruct dataset~\cite{liu2023visual} dataset, which is a set of GPT-generated multimodal instruction-following data.


\begin{table*}[ht]
\centering
   \adjustbox{max width=0.9\textwidth}{
    {\small
\begin{tabular}{c|l|c|ccccccc|c}
\toprule
\textbf{Model} & \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Wikitext2} & \textbf{Arc-Easy} & \textbf{Arc-Challenge} & \textbf{BoolQ} & \textbf{HellaSwag} & \textbf{OpenBookQA} & \textbf{WinoGrande} & \textbf{MMLU} & \textbf{Average} \\ \midrule
\multirow{8}{*}{\shortstack[c]{LLaMA‑3.2‑1B\\(2:4)}} & Dense & 9.06 & 65.36 & 31.40 & 63.82 & 47.73 & 26.60 & 60.69 & 31.19 & 46.68 \\ \cmidrule{2-11} 
 & Magnitude & 4808.42 & 27.95 & 19.45 & 38.50 & 26.13 & 11.80 & 51.78 & 23.80 & 28.49 \\
 & SparseGPT & \textbf{32.20} & \textbf{45.29} & 20.65 & 62.11 & \textbf{31.99} & 15.20 & 54.54 & 24.68 & \textbf{36.35} \\
 & Wanda & 75.76 & 37.16 & 18.17 & 62.05 & 28.57 & 12.00 & 50.20 & 24.45 & 33.23 \\
 & PrunerZero & 141.40 & 36.70 & 19.28 & 57.43 & 27.72 & 13.40 & 50.12 & 25.72 & 32.91 \\
 & CP & 68.17 & 38.35 & 18.14 & 62.08 & 28.56 & 12.40 & 53.31 & 23.82 & 33.81 \\
 & RIA & 72.56 & 38.12 & 20.33 & 61.34 & 27.12 & 12.80 & 52.76 & 24.31 & 33.83 \\
 & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}45.32 & \cellcolor{gray!20}42.27 & \cellcolor{gray!20}\textbf{21.08} & \cellcolor{gray!20}\textbf{62.12} & \cellcolor{gray!20}29.12 & \cellcolor{gray!20}\textbf{15.60} & \cellcolor{gray!20}\textbf{54.82} & \cellcolor{gray!20}\textbf{26.27} & \cellcolor{gray!20}35.90 \\ \midrule
\multirow{8}{*}{\shortstack[c]{LLaMA‑2‑7B\\(2:4)}} & Dense & 5.12 & 76.30 & 43.43 & 77.68 & 57.14 & 31.40 & 69.06 & 45.84 & 57.26 \\ \cmidrule{2-11} 
 & Magnitude & 52.00 & 61.87 & 30.20 & 59.79 & 45.42 & 21.80 & 60.93 & 26.87 & 43.84 \\
 & SparseGPT & 10.30 & 64.10 & \textbf{32.51} & \textbf{71.25} & \textbf{43.35} & \textbf{25.00} & \textbf{67.25} & \textbf{28.56} & \textbf{47.43} \\
 & Wanda & 11.38 & 62.75 & 30.38 & 67.65 & 41.18 & 23.60 & 62.59 & 27.82 & 45.14 \\
 & PrunerZero & 12.91 & 61.20 & 27.47 & 66.15 & 39.43 & 24.40 & 61.01 & 27.41 & 43.87 \\
 & CP & 10.68 & 63.32 & 30.96 & 66.92 & 41.32 & 23.80 & 63.56 & 26.51 & 45.20 \\
 & RIA & 10.52 & 63.67 & 31.82 & 67.13 & 42.03 & 23.00 & 64.13 & 27.56 & 45.62 \\
 & \cellcolor{gray!20}\textbf{Ours(Wanda)} & \cellcolor{gray!20}\textbf{10.17} & \cellcolor{gray!20}\textbf{64.22} & \cellcolor{gray!20}31.96 & \cellcolor{gray!20}68.17 & \cellcolor{gray!20}43.31 & \cellcolor{gray!20}23.60 & \cellcolor{gray!20}63.79 & \cellcolor{gray!20}28.13 & \cellcolor{gray!20}46.17 \\ \bottomrule
\end{tabular}}}
\caption{Comparisons of different pruning methods on the LLaMA3.2-1B and LLaMA2-7B language models. Performance across more sparsity patterns can be found in the supplementary materials.}
\label{tab:nlp_results}
\vspace{-4mm}
\end{table*}


%\begin{table*}[]
%\centering
%\resizebox{\textwidth}{!}{
%\begin{tabular}{c|l|c|ccccccc|c}
%\toprule
%\textbf{Model} & \multicolumn{1}{c|}{\textbf{Method}} & \textbf{Wikitext2} & \textbf{Arc-Easy} & \textbf{Arc-Challenge} & \textbf{BoolQ} & \textbf{HellaSwag} & \textbf{OpenBookQA} & \textbf{WinoGrande} & 


\subsubsection{Baselines.} Our method is compared with a variety of classic and state-of-the-art pruning baselines, including Magnitude~\cite{han2015learning}, Wanda \cite{sun2023wanda}, SparseGPT \cite{frantar2023sparsegpt}, PrunerZero~\cite{dong2024pruner}, CP \cite{pool2021channel}, and RIA \cite{zhangplug}.


\subsubsection{Evaluations.} %For vision model evaluations, we use the canonical \texttt{ImageNet-1K} validation dataset with top-1/5 accuracy as the primary metric. 
%For language model evaluations, we adopt perplexity as an evaluation metric to assess language comprehension ability, measured on the \texttt{WikiText2} test set~\cite{merity2016pointer}. To assess the effect of compression on a wide range of downstream tasks, we report zero-shot accuracy on \texttt{ARC}~\cite{allenai:arc}, \texttt{BoolQ}~\cite{clark2019boolq}, \texttt{HellaSwag}~\cite{zellers2019hellaswag}, \texttt{OpenBookQA}~\cite{OpenBookQA2018}, and \texttt{WinoGrande}~\cite{sakaguchi2021winogrande}, along with five-shot accuracy on the \texttt{MMLU} benchmark\cite{hendrycks2020measuring}.
%For multimodal evaluations, we report zero-shot \texttt{MMMU}~\cite{yue2024mmmu}, \texttt{MMStar}~\cite{chen2024we}, and \texttt{TextVQA}~\cite{singh2019towards} accuracy.

For vision evaluations, we use the standard \texttt{ImageNet-1K} validation set with top-1/5 accuracy as the main metric. 
For language models, we measure perplexity on the \texttt{WikiText2} test set~\cite{merity2016pointer} to assess language understanding. To evaluate compression effects across tasks, we report zero-shot accuracy on \texttt{ARC}~\cite{allenai:arc}, \texttt{BoolQ}~\cite{clark2019boolq}, \texttt{HellaSwag}~\cite{zellers2019hellaswag}, \texttt{OpenBookQA}~\cite{OpenBookQA2018}, and \texttt{WinoGrande}~\cite{sakaguchi2021winogrande}, along with five-shot accuracy on \texttt{MMLU}~\cite{hendrycks2020measuring}.
For multimodal tasks, we report zero-shot accuracy on \texttt{MMMU}~\cite{yue2024mmmu}, \texttt{MMStar}~\cite{chen2024we}, and \texttt{TextVQA}~\cite{singh2019towards}.


\subsubsection{Implementation Details.}
We use Wanda as our mask generator by default. Vision models are trained for 20 epochs on 2 AMD MI250 GPUs with AdamW (weight decay $0.01$, base learning rate $0.1$) under a cosine decay schedule and no warm-up, which takes around 4 hours.  Language models and vision-language models are trained for 20 and 10 update epochs, respectively, with AdamW ($\text{lr}=10^{-4}$). Training takes approximately 10 hours for a 1B model and 40 hours for a 7B model. The default permutation group number $G$ is 4. All runs use native AMP with FP16 precision, gradient accumulation set to one, and a small Smooth-L1 distillation term weighted $10^{-5}$. The default N:M sparsity is 2:4. 

\subsection{Comparison with State-of-the-Art Methods on Different Transformers}

\subsubsection{Results on Vision Transformers.}
%On the vision side, we apply structured pruning to \texttt{ViT-Base/16} and \texttt{ViT-Large/14} under the 2:4 and 4:8 sparsity patterns, retaining 50\% of the weights. Across all settings, our method consistently achieves the highest top-1 and top-5 accuracy among the compared approaches. For \texttt{ViT-Base/16}, our method obtains 67.9\% / 87.9\% (top-1 / top-5) accuracy at 2:4 sparsity, outperforming the strongest baseline (RIA) by 1.3\%age points. At 4:8 sparsity, it further improves to 71.8\% / 90.2\%, slightly ahead of RIA by 0.4 and 0.3 points. Similar trends are observed on \texttt{ViT-Large/14}, where our method reaches 80.7\% / 95.8\% at 2:4 sparsity and 82.7\% / 96.5\% at 4:8 sparsity, both surpassing prior methods. These results highlight the effectiveness of our approach in preserving accuracy for Vision Transformers. 

On the vision side, we apply structured pruning to \texttt{ViT-Base/16} and \texttt{ViT-Large/14} under 2:4 and 4:8 sparsity, retaining 50\% of weights. Our method consistently achieves the highest top-1 and top-5 accuracy across all settings. For \texttt{ViT-Base/16}, it reaches 67.9\% / 87.9\% (top-1 / top-5) at 2:4 sparsity, outperforming the strong permutation baseline (RIA) by 1.3 points. At 4:8 sparsity, accuracy improves to 71.8\% / 90.2\%, slightly ahead of RIA by 0.4 / 0.3 points. Similar gains are observed on \texttt{ViT-Large/14}, achieving 80.7\% / 95.8\% at 2:4 and 82.7\% / 96.5\% at 4:8 sparsity, both surpassing prior permutation methods. These results demonstrate the accuracy-preserving strength of our approach on Vision Transformers.


\begin{table}[ht]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{9pt}
  {\renewcommand{\arraystretch}{1.02}%
   \setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{1pt}%
      \adjustbox{max width=0.45\textwidth}{
    {\small
   \begin{tabular}{@{}c|l|ccc|c@{}}
    \toprule
    Sparsity & Method & MMMU & MMStar & TextVQA & Average \\
    \midrule
    0\% & Dense & 53.1 & 55.8 & 79.3 & 62.7 \\
    \cmidrule{1-6}
    \multirow{4}{*}{2:4}
      & Magnitude & 34.1 & 48.7 & 76.5 & 53.1 \\
      & Wanda     & 37.2 & 51.2 & 77.2 & 55.2 \\
      & RIA       & 37.3 & 51.4 & 77.1 & 55.3 \\
      & \cellcolor{gray!20}\textbf{Ours(Wanda)}
        & \cellcolor{gray!20}\textbf{38.1}
        & \cellcolor{gray!20}\textbf{51.9}
        & \cellcolor{gray!20}\textbf{77.8}
        & \cellcolor{gray!20}\textbf{55.9} \\
    \bottomrule
   \end{tabular}%
   }
   }
  }
  \vspace{-2mm}
  \caption{Performance of Qwen2.5-VL-3B under different pruning methods.}
  \label{tab:mmmu_pruning}
  \vspace{-4mm}
\end{table}

\begin{table}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{9pt}
  {\renewcommand{\arraystretch}{1.02}%
   \setlength{\aboverulesep}{0pt}\setlength{\belowrulesep}{1pt}%
      \adjustbox{max width=0.45\textwidth}{
    {\small
   \begin{tabular}{@{}c|c|ccc|c@{}}
    \toprule
    Epochs & Wikitext2 & Arc-Easy & Arc-Chall. & MMLU & Average \\
    \midrule
      0  & 11.38 & 62.75 & 30.38 & 27.82 & 40.32 \\
      1  & 10.56 & 62.89 & 30.92 & 27.61 & 40.47 \\
      2  & 10.31 & 63.15 & 31.02 & 27.96 & 40.71 \\
      5  & 10.27 & 64.10 & 31.92 & 28.05 & 41.36 \\
     10  & 10.21 & \textbf{64.23} & 31.88 & 28.12 & 41.41 \\
     \cellcolor{gray!20}20  & \cellcolor{gray!20}\textbf{10.17} & \cellcolor{gray!20}64.22 & \cellcolor{gray!20}\textbf{31.96} & \cellcolor{gray!20}\textbf{28.13} & \cellcolor{gray!20}\textbf{41.44} \\
    \bottomrule
   \end{tabular}%
   }
   }
  }
  \vspace{-2mm}
  \caption{Performance of our approach on LLaMA‑2‑7B with different training epochs.}
  \label{tab:epoch_results}
  \vspace{-4mm}
\end{table}

\subsubsection{Results on Language Transformers.}
On the language side, we evaluate pruning performance on both \texttt{LLaMA-3.2-1B} and \texttt{LLaMA-2-7B} models across a range of context modeling and commonsense benchmarks. Our method—using Wanda pruning followed by a learned channel permutation—consistently improves downstream performance over baseline methods without requiring weight updates. On \texttt{LLaMA-3.2-1B}, our approach improves the average accuracy to 35.90\%, outperforming Wanda (33.23\%), CP (33.81\%), and RIA (33.83\%) by 2.1 to 2.7 points. Similar trends are observed on \texttt{LLaMA-2-7B}, where our method reaches 46.17\% average accuracy, compared to 45.14\% (Wanda), 45.20\% (CP), and 45.62\% (RIA). Notably, our method improves performance on challenging tasks such as \texttt{ARC-Challenge} (e.g., +3.79 points over Wanda for LLaMA-3.2-1B) and maintains strong results on \texttt{BoolQ} and \texttt{WinoGrande}. While methods like SparseGPT achieve higher accuracy due to weight updates, our approach operates in the same constrained setting as Wanda, offering a fair and efficient comparison. Moreover, on \texttt{WikiText2}, our method yields significantly better perplexity than SparseGPT and PrunerZero, demonstrating its ability to preserve language modeling quality after pruning. %under structured sparsity.

\subsubsection{Results on Multimodal Transformers.}
As shown in Table~\ref{tab:mmmu_pruning}, our method achieves the highest performance among all evaluated 2:4 structured pruning approaches on the \texttt{MMMU} benchmark using the \texttt{Qwen2.5-VL-3B} model. While traditional methods such as Magnitude pruning and recent techniques like Wanda and RIA yield scores of 34.1, 37.2, and 37.3 respectively, our approach outperforms them with a score of 37.9, demonstrating its effectiveness in preserving critical information under structured sparsity constraints. 


For Transformer-based models of various types, the learnable permutation consistently lifts performance beyond magnitude-only or rule-based permutation strategies, and does so while preserving the full latency advantage of $2{:}4$ sparsity.  %The effect is especially pronounced on benchmarks that rely on multi-step reasoning, suggesting that permutation learning helps concentrate semantically aligned features into the survivable positions of each weight block.

% ------------------------------------------------------------------
% Vision results (ImageNet, ViT-Base/16)
% ------------------------------------------------------------------

%\begin{table}[t]
%\centering
%\caption{Top-1 accuracy on ImageNet after pruning ViT-Base/16 to the $2{:}4$ structured pattern
%(50\,\% non-zero weights).}
%\label{tab:vit_results}
%\begin{tabular}{lcc}
%\toprule
%\textbf{Method} & \textbf{Sparsity (\%)} & \textbf{Top-1 (\%)} \\
%\midrule
%Dense baseline & 0 & 82.1 \\
%Channel Pruning (CP) & 50 & 66.5 \\
%Recurrent Importance Allocation (RIA) & 50 & 66.8 \\
%\textbf{Ours: Wanda + learn2perm} & 50 & \textbf{67.4} \\
%\bottomrule
%\end{tabular}
%\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



% Please add the following required packages to your document preamble:
% 





\begin{table*}[ht]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
    \adjustbox{max width=0.9\textwidth}{
    {\small
  \begin{tabular}{@{}c|c|c|c c c c c c c|c@{}}
    \toprule
    Number of Group & Trainable Parameters & Wikitext2 & Arc‑Easy & Arc‑Chall. & BoolQ & HellaSwag & OpenBookQA & WinoGrande & MMLU & Average \\
    \midrule
      1  & $1.0 \times$   & 10.11 & 64.89 & 32.04 & 68.02 & 43.56 & 23.80 & 63.92 & 28.07 & 46.33 \\
      2  & $0.68\times$    & 10.12 & 64.35 & 31.84 & 68.21 & 43.82 & 23.60 & 64.02 & 28.25 & 46.30 \\
  \rowcolor{gray!20}
      4  & $0.41\times$  & 10.17 & 64.22 & 31.96 & 68.17 & 43.31 & 23.60 & 63.79 & 28.13 & 46.17 \\
      8  & $0.23\times$   & 10.25 & 64.15 & 31.82 & 68.21 & 43.15 & 23.60 & 63.82 & 28.15 & 46.13 \\
     16  &   $0.12\times$  & 10.63 & 63.59 & 31.15 & 67.92 & 42.89 & 23.00 & 63.72 & 27.67 & 45.71 \\
    \bottomrule
  \end{tabular}
  }
  }
  \caption{Performance of our approach on LLaMA‑2‑7B with different permutation group numbers.}
  \label{tab:group_results}

\end{table*}




\begin{table*}[ht]
  \centering
  \footnotesize
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.15}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{@{}l|l|c|c c c c c c c|c@{}}
    \toprule
    Model & Pruning Methods & Wikitext2(Ours/Baseline) & Arc‑Easy & Arc‑Chall. & BoolQ & HellaSwag & OpenBookQA & WinoGrande & MMLU & Average(Ours/Baseline) \\
    \midrule
    \multirow{4}{*}{LLaMA‑2‑7B}
      & Magnitude(Ours)    & 45.82 /52.00 & 62.89 & 30.90 & 61.68 & \textbf{45.47} & 22.20 & 62.12 & 27.12 & 44.63 /43.84 \\
      & Wanda(Ours)        & 10.17/11.38 & 64.22 & 31.96 & 68.17 & 43.31 & 23.60 & 63.79 & 28.13 & 46.17/45.14 \\
      & RIA(Ours)          & 10.02/10.52 & 63.88 & 32.53 & \textbf{68.83} & 42.59 & 24.00 & 64.32 & 29.02 & 46.45/45.62 \\
      &\cellcolor{gray!20}AdmmPruner(Ours)   &  \cellcolor{gray!20}\textbf{9.56}/9.68 & \cellcolor{gray!20}\textbf{69.02} & \cellcolor{gray!20}\textbf{32.68} & \cellcolor{gray!20}63.41 & \cellcolor{gray!20}45.12 & \cellcolor{gray!20}\textbf{26.00} & \cellcolor{gray!20}\textbf{65.96} & \cellcolor{gray!20}\textbf{29.62} & \cellcolor{gray!20}\textbf{47.40}/47.05 \\
    \bottomrule
  \end{tabular}}
  \caption{Performance of different pruning methods when integrated with our approach on LLaMA‑2‑7B.}
  \label{tab:more_baselines}
  \vspace{-4mm}
\end{table*}

\begin{table}[H]
  \centering
  
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l|c|c|c|c|c@{}}
      \toprule
      Loss & Wikitext2 & Arc‑Easy & Arc‑Chall. &  MMLU & Average \\
      \midrule
      %Pres.\_mag\_sum           & 568.72 & 30.25 & 19.56 &  23.96 & 24.59 \\
      %Pres.\_wanda\_metric\_sum & 62.14  & 39.43 & 18.83 &  25.71 & 27.99 \\
      %Pres.\_ria\_metric\_sum   & 65.43  & 38.91 & 19.89 &  25.19 & 28.00 \\
      CE Loss                   & 46.15  & 42.01 & 20.53 &  26.12 & 29.55 \\
      Distillation Loss              & 52.58  & 40.51 & 20.12 &  25.97 & 28.87 \\
      \cellcolor{gray!20}CE+Distillation loss           & \cellcolor{gray!20}\textbf{45.32}  & \cellcolor{gray!20}\textbf{42.27} & \cellcolor{gray!20}\textbf{21.08} &  \cellcolor{gray!20}\textbf{26.27} & \cellcolor{gray!20}\textbf{29.87} \\
      \bottomrule
    \end{tabular}}
    \caption{Ablation study of our optimzation loss on LLaMA3.2-1B across benchmarks.}
  \label{tab:loss}
  \vspace{-4mm}
\end{table}


\subsection{Training Convergence and Efficiency}
To assess convergence, we report performance from epoch 1 to 20 in Table~\ref{tab:epoch_results}. The initial performance is limited (average 33.23; \texttt{Wikitext2} perplexity 75.76), but improves markedly after one epoch, reaching 40.47 and 10.56 respectively, reflecting an 86\% reduction in perplexity and indicating fast optimization of the permutator. Subsequent gains taper off: 40.71 at epoch 2, 41.36 at epoch 5, 41.41 at epoch 10, and 41.44 at epoch 20.
Task-level improvements show a similar pattern. \texttt{Arc‑Easy} improves from 37.16 to 64.22, \texttt{Arc‑Challenge} from 18.17 to 31.96, and \texttt{MMLU} from 24.45 to 28.13, with most gains observed after the first epoch, which takes approximately 3 to 4 hours.

We also evaluate other heuristic permutation methods under the same settings, such as the LSA algorithm in RIA and the search-based approach in CP. These methods typically require 5 to 10 times longer to converge compared to our approach. These results suggest that the method converges efficiently, with nearly all achievable performance obtained within five epochs, only 0.08 below the final result at epoch 20, while maintaining low per-epoch computational cost.




%To assess training convergence, we track performance from the very start of training (epoch 1) to 20 epochs, as shown in Table~\ref{tab:epoch_results}. The initial point is weak (average 33.23, \texttt{Wikitext2} perplexity 75.76), but after just one epoch the average jumps to 40.47 and perplexity drops to 10.56, an approximately 86\% reduction, showing the permutator is extremely fast to optimize. Longer training continues to help but with clear saturation: 40.71 at 2 epochs, 41.36 at 5, 41.41 at 10, and 41.44 at 20. Across tasks, \texttt{Arc‑Easy} improves from 37.16 to 64.22, \texttt{Arc‑Challenge}. from 18.17 to 31.96, and \texttt{MMLU} from 24.45 to 28.13, with most gains already achieved in the first epoch, which takes 3 to 4 hours approximately.
%Overall, the results highlight the rapid convergence and training efficiency of our method: nearly all attainable accuracy is achieved within just five epochs—only 0.08 below the performance at 20 epochs—making it an ideal default. Moreover, each epoch is computationally lightweight, further underscoring the method’s suitability for efficient training.


\subsection{Ablation Study}

\subsubsection{Impact of Permutation Group Number.}
%We study how the number of permutation groups $G$ (i.e., how finely we partition a weight matrix before learning permutations) influences both effectiveness and efficiency. A smaller $G$ (larger groups) allows the permutator to explore more global reorderings, which should yield better permutation masks. A larger $G$ (smaller groups) shrinks the learnable permutator, reducing parameters, but also constrains the search space.

We investigate how the number of permutation groups $G$, defined as the granularity of partitioning the weight matrix before learning permutations, affects performance and efficiency. A smaller $G$ enables more global reordering, potentially leading to better permutation masks. A larger $G$ reduces the number of parameters but constrains the search space. As shown in Table~\ref{tab:group_results}, we evaluate $G \in \{1, 2, 4, 8, 16\}$ on \textsc{LLaMA‑2‑7B}.
The average score decreases only marginally from 46.33 at $G=1$ to 46.30, 46.17, 46.13, and 45.71 as the number of groups increases. \texttt{Wikitext2} perplexity rises slightly from 10.11 to 10.63. Meanwhile, the number of trainable parameters is significantly reduced.
 Considering the reduced number of trainable parameters, along with the preservation of \texttt{Wikitext2} perplexity and task accuracy, we adopt $G=4$ as the default setting in this paper. Notably, $G=8$ is also a viable option when a bigger accuracy drop is acceptable and computational resources are limited.
 %The largest task drop is on Arc‑Easy (64.89 to 63.59). Between G=4 and 8 the average differs by just 0.04, showing diminishing returns once moderate group sizes are allowed.
%The permutator's parameter count and training time shrink roughly in proportion to the number of groups. Moving from G=1 to 4 cuts the cost by about 16$\times$ for only a 0.16 drop in the average score, while G=2 is almost identical to G=1 (-0.03). We therefore adopt G=4 as the default in the rest of the paper.

%On the other hand, trainable parameters are 51.31\% for group 1, 34.92\% for group 2, 20.85\% for group 4, 11.64\% for group 8, and 6.18\% for group 16, while wall clock time is about 4 hours for groups 1 to 4, about 6 hours for group 8, and about 9 hours for group 16. Relative to group 1, group 4 reduces trainable parameters by about 59\% with essentially unchanged average score from 46.33 to 46.17 and no extra time; moving to groups 8 and 16 cuts parameters further but changes the average score by only 0.04 and 0.46 while increasing time by about 50\% and 125\%. We therefore adopt group 4 by default.



\subsubsection{Performance over Different Pruning Methods.}
%To assess the generality of our approach, we incorporate the learnable permutator into four distinct pruning baselines: Magnitude, Wanda, RIA, and AdmmPruner. As shown in Table~\ref{tab:more_baselines}, our method consistently improves performance across all cases. Specifically, the average score of Magnitude increases from 43.84 to 44.63, Wanda from 45.14 to 46.17, and RIA from 45.62 to 46.45. Wikitext2 perplexity is reduced in every case—for instance, from 52.00 to 45.82 for Magnitude, from 11.38 to 10.17 for Wanda, and from 10.52 to 10.02 for RIA. On MMLU, the scores improve from 26.87, 27.82, and 27.56 to 27.12, 28.13, and 29.02, respectively. Moreover, our permutator is compatible with post-pruning weight updates: when combined with AdmmPruner, it achieves the highest overall average (47.40), the best MMLU score (29.62), and the lowest Wikitext2 perplexity (9.56). These results demonstrate that the proposed permutator is broadly applicable and complementary to existing pruning strategies and post-pruning optimization techniques.

To assess the generality of our approach, we integrate the learnable permutator into four representative pruning baselines: Magnitude, Wanda, RIA, and AdmmPruner. As shown in Table~\ref{tab:more_baselines}, our method consistently enhances performance across all settings. Specifically, the average score improves from 43.84 to 44.63 for Magnitude, from 45.14 to 46.17 for Wanda, and from 45.62 to 46.45 for RIA. The perplexity on \texttt{Wikitext2} also decreases in every case—for example, from 52.00 to 45.82 for Magnitude, from 11.38 to 10.17 for Wanda, and from 10.52 to 10.02 for RIA. On \texttt{MMLU}, the scores rise from 26.87, 27.82, and 27.56 to 27.12, 28.13, and 29.02, respectively.

Furthermore, the permutator is compatible with post-pruning weight updates. When applied to AdmmPruner, it achieves the highest overall average score (47.40), the best \texttt{MMLU} accuracy (29.62), and the lowest \texttt{Wikitext2} perplexity (9.56). These results demonstrate that the proposed permutator is broadly applicable and complementary to both pruning baselines and post-pruning optimization techniques.


\subsubsection{Effect of Our Optimization Loss.}
%To understand how to train the permutator, we compare indirect objectives that try to preserve weight statistics with end to end objectives that optimize the model outputs directly. Table \ref{tab:loss} shows that the indirect objectives are clearly weaker: preserved magnitude reaches an average of 31.37 with a very high Wikitext2 perplexity of 568.72, while the Wanda and RIA metric sums reach 33.96 and 34.09. In contrast, end to end signals are consistently better.
%To assess the individual and combined contributions of our proposed optimization components, namely the end-to-end cross-entropy (CE) loss and the layer-wise distillation loss, we perform an ablation study.
%As shown in Table~\ref{tab:loss}, using only the end-to-end cross-entropy loss yields an average score of 29.55 with a substantially reduced perplexity of 46.15, while the layer-wise distillation loss alone achieves an average of 28.87. When combined, the two losses produce the best overall performance: an average score of 29.87, with the highest results on \texttt{Arc‑Easy} (42.27), \texttt{Arc‑Challenge} (21.08),  and \texttt{MMLU} (26.27), along with a competitive perplexity of 45.32.
%These results suggest that both the cross-entropy and layer-wise distillation losses provide meaningful supervision, and their combination offers the most consistent and reliable improvements across tasks.

%To evaluate the contributions of our optimization components—end-to-end cross-entropy (CE) loss and layer-wise distillation—we conduct an ablation study. As shown in Table~\ref{tab:loss}, CE loss alone achieves an average score of 29.55 and perplexity of 46.15, while distillation alone yields 28.87. Their combination leads to the best results: an average score of 29.87 with top performance on \texttt{Arc‑Easy} (42.27), \texttt{Arc‑Challenge} (21.08), and \texttt{MMLU} (26.27), and a low perplexity of 45.32. These findings confirm the complementary benefits of both loss terms.

To evaluate the contributions of our optimization components end-to-end cross entropy (CE) loss and layer wise distillation we conduct an ablation study. As shown in Table~\ref{tab:loss}, CE loss alone achieves an average score of 29.55 and perplexity of 46.15, while distillation alone yields 28.87. Their combination leads to the best results: an average score of 29.87 with top performance on Arc Easy (42.27), Arc Challenge (21.08), and MMLU (26.27), and a low perplexity of 45.32. These findings confirm the complementary benefits of both loss terms.

%As shown in Table~\ref{tab:loss},
%end-to-end cross-entropy loss attains an average of 35.66 with a much lower perplexity of 46.15, and the layer wise distillation loss reaches 34.86. Using both together yields the best overall result: an average of 36.11, the strongest scores on Arc Easy (42.27), Arc Challenging (21.08), WinoGrande (54.82), and MMLU (26.27), and a competitive perplexity of 45.32. These observations indicate that indirect weight based heuristics are insufficient for steering the permutation, while both cross entropy and layer wise distillation effectively guide learning, and their combination provides the most reliable gains.





==> sections/introduction.tex <==
\section{Introduction}
Transformers have emerged as the cornerstone architecture in modern deep learning, driving breakthroughs across a broad spectrum of AI tasks. In computer vision, models such as Vision Transformer (ViT)~\cite{yuan2021tokens}, DETR~\cite{carion2020end}, and DiT~\cite{peebles2023scalable} have demonstrated that transformer-based designs can outperform previous architectures in tasks like image classification, object detection, and generative modeling (diffusion). In natural language processing, large language models (LLMs) such as GPT~\cite{floridi2020gpt}, LLaMA~\cite{touvron2023llama}, Qwen~\cite{bai2023qwen}, and DeepSeek~\cite{guo2025deepseek} have pushed the boundaries of context understanding, text generation, and complex reasoning. The architectural flexibility and strong inductive capabilities of transformers have made them the de facto choice for foundation models across modalities.

This widespread adoption, however, comes at a significant cost when deploying transformer-based models on resource-constrained devices, due to the rapid—and often exponential—growth in model size. Recent LLMs, for instance, often comprise hundreds of billions of parameters, rendering inference computationally intensive and economically prohibitive. To address the escalating complexity of transformer models, various acceleration techniques have been proposed, such as pruning {\textcolor{red}{[3-CITE]}}, quantization {\textcolor{red}{[3-CITE]}}, and knowledge distillation{\textcolor{red}{~\cite{gou2021knowledge}}}. Structured sparsity, often referred to as N:M sparsity, enforces that within every group of M consecutive weights, at most N are non-zero. This regular sparsity pattern not only reduces parameter count but also aligns well with modern hardware (e.g. Sparse Tensor Cores in recent GPU architectures for 2:4 sparsity). As a result, structured sparsity is both practical and suitable for real-world deployment.

% This widespread adoption, however, comes with a significant cost when deploying transformer-based models in edge devices: the rapid and often exponential increase in model size. For example, recent LLMs are routinely composed of hundreds of billions of parameters, making training and inference computationally intensive and economically challenging. 
% Consequently, efficient model deployment—especially on edge devices or in latency-sensitive applications—has become a critical bottleneck. These practical constraints have sparked a growing interest in model compression and acceleration techniques aimed at reducing resource consumption without compromising performance, motivating the development of lightweight, scalable alternatives to vanilla transformer architectures~\cite{tay2022efficient,narang2021transformer}.
% To cope with the growing complexity of transformer-based models, a range of model acceleration techniques have been explored. Among the most widely used are pruning, quantization, and knowledge distillation~\cite{gou2021knowledge}. Structured pruning, in particular, has gained popularity due to its hardware-friendliness and compatibility with efficient inference engines. A commonly used structured sparsity pattern is (M, N)-sparsity~\cite{zhou2021learning}, where within every M consecutive weights, at most N are retained as non-zero. This sparsity constraint enables predictable memory access and parallel computation, making it preferable over unstructured sparsity in practical deployment.

Several recent methods, such as Wanda~\cite{sun2023simple}, SparseGPT~\cite{frantar2023sparsegpt}, and Pruner-Zero {\textcolor{red}{[CITE]}}, leverage structured sparsity to compress large-scale models with controllable accuracy degradation. However, a key challenge in further improving post-sparsification performance lies in the rigid coupling between the weight layout and the imposed sparsity pattern. To address this, weight permutation~\cite{pool2021channel} has emerged as an effective auxiliary strategy. By reordering the channels of the weight matrix prior to pruning, weight saliencies can be more uniformly redistributed to better match the imposed sparsity pattern, thereby reducing post-pruning accuracy loss. Owing to the combinatorial complexity of the permutation space, current methods often rely on heuristic or greedy solutions~\cite{zhangplug}, thereby restricting the achievable gains from reordering. 


To overcome these limitations, we propose an \textbf{end-to-end learnable} framework to optimize weight permutation for structured pruning of Transformer-based models. Our method introduces three main contributions as follows:

\begin{itemize}
    \item A \textbf{learnable permutation cost matrix} that explicitly quantifies the cost of swapping any two input channels of a given weight matrix.
    \item To address the non-differentiability of discrete permutation, we design a \textbf{differentiable approximation of bipartite matching} guided by the learnable cost matrix, enabling efficient and accurate binary permutation matrix learning with minimal computational overhead.
    \item A \textbf{sparsity-aware} {\textcolor{red}{[I can not see sparsity aware]}} loss function is proposed to jointly guide the optimization of the permutation operator, achieving a fine balance between task-specific performance and alignment with the dense teacher model through knowledge distillation.
\end{itemize}

Through end-to-end learning, the proposed framework derives a dedicated permutation matrix for each weight tensor, which is then multiplied with the original weights to produce reordered weights that aligns more naturally with the target sparsity pattern.
We apply this approach to both vision and language models, including ViT, LLM, and VLM backbones, and conduct extensive experiments to validate its effectiveness. Experimental results demonstrate that our framework achieves state-of-the-art structured sparsity with significantly reduced accuracy degradation, outperforming traditional greedy baselines on a variety of benchmarks.

==> sections/introduction_v2.tex <==
\section{Introduction}
Transformers have emerged as the cornerstone architecture in modern deep learning, driving breakthroughs across a broad spectrum of AI tasks. In computer vision, models such as Vision Transformer (ViT)~\cite{yuan2021tokens}, DETR~\cite{carion2020end}, and DiT~\cite{peebles2023scalable} have demonstrated that Transformer-based designs can outperform previous architectures in tasks like image classification, object detection, and generative modeling (diffusion). In natural language processing, large language models (LLMs) such as GPT~\cite{floridi2020gpt}, LLaMA~\cite{touvron2023llama}, Qwen~\cite{bai2023qwen}, and DeepSeek~\cite{guo2025deepseek} have pushed the boundaries of context understanding, text generation, and complex reasoning. The architectural flexibility and strong inductive capabilities of Transformers have made them the de facto choice for foundation models across modalities.

The widespread adoption of Transformer-based models, however, comes at a significant cost when deploying them on resource-constrained devices, due to the rapid—and often exponential—growth in model size. Recent LLMs, for instance, often comprise hundreds of billions of parameters, rendering inference computationally intensive and economically prohibitive. To address the escalating complexity of Transformer models, various acceleration techniques have been proposed, such as pruning~\cite{zhao2024apt,ma2023llm,men2024shortgpt}, quantization~\cite{lin2024awq,xiao2023smoothquant,liu2024spinquant}, and knowledge distillation~\cite{gu2023minillm}. Structured sparsity, also referred to as N:M sparsity, enforces that within every group of M consecutive weights, at most N are non-zero. This regular sparsity pattern not only reduces parameter count but also aligns well with modern hardware (e.g. Sparse Tensor Cores in recent GPU architectures for 2:4 sparsity). As a result, structured sparsity is both practical and suitable for real-world deployment.


Several recent methods, such as Wanda~\cite{sun2023simple}, SparseGPT~\cite{frantar2023sparsegpt}, and Pruner-Zero~\cite{dong2024pruner}, leverage structured sparsity to prune large-scale models with controllable accuracy degradation. However, a key challenge in further improving post-pruning performance lies in the rigid coupling between the weight layout and the imposed sparsity pattern. To address this, weight permutation~\cite{pool2021channel} has emerged as an effective auxiliary strategy. By reordering the channels of the weight matrix prior to pruning, weight saliencies can be more uniformly redistributed to better match the imposed sparsity pattern, thereby reducing post-pruning accuracy loss. Owing to the increasingly combinatorial complexity of the permutation space in large-scaled Transformer-based models, current methods often rely on heuristic or greedy solutions~\cite{zhangplug}, thereby restricting the achievable gains from reordering. 


To overcome these limitations, we propose an \textbf{end-to-end learnable} framework to optimize weight permutation for structured pruning of Transformer-based models. Our method introduces three main contributions as follows:

\begin{itemize}
    \item A \textbf{learnable permutation cost matrix} that explicitly quantifies the cost of swapping any two input channels of a given weight matrix.
    \item To address the non-differentiability of discrete permutation, we design a \textbf{differentiable approximation of bipartite matching} guided by the learnable cost matrix, enabling efficient and accurate binary permutation matrix learning with minimal computational overhead.
    \item A \textbf{sparsity optimization loss} function is proposed to jointly guide the optimization of the permutation operator, achieving a fine balance between task-specific performance and alignment with the dense teacher model through knowledge distillation.
\end{itemize}

Through end-to-end learning, the proposed framework derives a dedicated permutation matrix for each weight tensor, which is then multiplied with the original weights to produce reordered weights that aligns more naturally with the target sparsity pattern.
We apply this approach to both vision and language models, including ViT, LLM, and VLM backbones, and conduct extensive experiments to validate its effectiveness. Experimental results demonstrate that our framework achieves state-of-the-art structured sparsity with significantly reduced accuracy degradation, outperforming traditional greedy baselines on a variety of benchmarks.

==> sections/methods.tex <==
\section{Methods}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{Figures/perm_isbetter.pdf} 
\caption{The channel permutation process enhances the friendliness of the 2:4 sparsification, making the overall saliency of the pruning metric more preserved.}
\label{fig:channel-perm}
\end{figure}


In this section, we first introduce some preliminaries about channel permutation for N:M pruning Transformers. We then present our novel end-to-end learnable permutation framework, which incorporates a learnable permutation cost matrix, a differentiable bipartite matching solver, and a sparsity optimization loss function to directly optimize the permutation operator for both vision transformers and large language models.


\subsection{Preliminaries}
\label{sec:preliminaries}

\subsubsection{Channel Permutation for N:M Sparsity.} Channel permutation is an effective technique for enhancing the compatibility of neural network weights with structured sparsity patterns, such as 2:4 sparsity. As illustrated in Figure~\ref{fig:channel-perm}, the original weight layout may exhibit an uneven distribution of the saliency metric, where high or low values are concentrated within certain blocks. This non-uniformity poses challenges for fixed sparsity patterns to retain the most informative weights, often resulting in a lower overall saliency after pruning.

By applying channel permutation prior to pruning, saliency values can be redistributed more uniformly across blocks. This increases the likelihood that each 4-element group contains a representative mix of salient and non-salient weights, thereby improving the effectiveness of 2:4 sparsification. Consequently, more critical weights are preserved, leading to better retention of salient information in the pruned model.

\subsubsection{Channel Permutation for Linear Layers.} When applying a channel permutation to the input dimension of the weight matrix in a linear layer, it is essential to maintain output consistency by ensuring that the corresponding input activation is permuted in the same manner. Specifically, if a permutation matrix \( \mathbf{P} \) is applied to the input channels of the \( i \)-th layer’s weight matrix \( \mathbf{W}^{\top}_i  \in \mathbb{R}^{d_\text{in} \times d_\text{out}}\), i.e., \( \hat{\mathbf{W}}_{i}^{\top} = \mathbf{P} \mathbf{W}^{\top}_i\), then the input dimension of its activation \( \mathbf{A}_i \in \mathbb{R}^{d_\text{batch} \times d_\text{in}} \) must also be permuted as \( \hat{\mathbf{A}}_i = \mathbf{A}_i\mathbf{P}^{\top} \) to preserve the computation: \( \mathbf{\hat{A}}_{i+1} = \mathbf{\hat{A}}_{i}\mathbf{\hat{W}}^{\top}_{i+1} =\mathbf{A}_i\mathbf{P}^{\top}\mathbf{P} \mathbf{W}^{\top}_i  =\mathbf{A}_i \mathbf{W}^{\top}_i=\mathbf{A}_{i+1}\) ($\mathbf{P}^{\top} = \mathbf{P}^{-1}$). To avoid the computational cost of explicitly permuting activations at runtime, we can instead permute the output channels of the preceding \((i{-}1)\)-th layer’s weight matrix (\( \hat{\mathbf{W}}_{i-1} = \mathbf{W}_{i-1} \mathbf{P}^{\top} \)) to make \( \hat{\mathbf{A}}_{i} = \mathbf{A}_{i-1}\hat{\mathbf{W}}_{i-1} = \mathbf{A}_{i}\mathbf{P}^{\top}\), as shown in Figure~\ref{fig:perm_between_layers}. This strategy preserves functional equivalence while eliminating the need for activation reordering.


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm_between_layers.pdf} 
\caption{To guarantee output consistency, after the input channel of the $i$-th layer weight is permuted, the input activation of that layer should also be permuted accordingly, which can be realized by permuting the output channel of the previous $i-1$-th layer weight accordingly.}
\label{fig:perm_between_layers}
\end{figure}

\subsubsection{Channel Permutation for Transformers.} Transformer architecture goes far beyond sequential linear layers. As shown in Figure~\ref{fig:transformer_perm}, a typical Transformer block comprises two principal functional modules: a multi-head self-attention mechanism (MHA) and a feed-forward network (FFN). Given the incoming representation \( \mathbf{X}_{i-1} \) at layer \( i \), the transformed output \( \mathbf{X}_{i} \) is computed through this sequence of operations:

\begin{equation}
\label{eq:1}
\begin{aligned}
    \mathbf{A} &= \text{LayerNorm}\left(\mathbf{A}_{i-1} + \operatorname{MHA}(\mathbf{A}_{i-1})\right), \\
    \mathbf{A}_i &= \text{LayerNorm}\left(\mathbf{A} + \mathrm{FFN}(\mathbf{A})\right).
\end{aligned}
\end{equation}

In the multi-head self-attention (MHA) module, the projection matrices \( \mathbf{W}_q \), \( \mathbf{W}_k \), and \( \mathbf{W}_v \) map the same input into query, key, and value representations, respectively, and thus share a common input channel structure. To maintain their functional alignment, any channel permutation must be applied jointly to all three matrices. Moreover, when doing input channel permutation for the mapping weight $\mathbf{W}_o$ for attention output, \( \mathbf{W}_q \), \( \mathbf{W}_k \), and \( \mathbf{W}_v \) should also do the corresponding output channel permutation in an aggregated manner. The feed-forward network (FFN) follows a similar structure: \( \mathbf{W}_{up} \) and \( \mathbf{W}_{gate} \) operate on the same input and must share the same permutation, while their output permutation must align with the input of the down-projection matrix \( \mathbf{W}_{down} \). Therefore, channel permutation must be designed and applied in a structured, group-wise manner to preserve the internal consistency of MHA and FFN submodules. A detailed theoretical justification for these constraints is provided in Appendix~X.


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/transformer_perm.pdf} 
\caption{An overview of channel permutation for Transformer layers. $W_q$, $W_k$, and $W_v$ need to learn their input channel permutation in an aggregated way and make corresponding adjustments in their output channel for $W_o$'s input channel permutation. $W_{gate}$ and $W_{up}$ are congruent.}
\label{fig:transformer_perm}
\end{figure}

% \noindent \textbf{Structural Sparsity.} Structural sparsity has emerged as a promising approach to reduce the computational and memory overhead of deep neural networks while retaining hardware efficiency. Among various forms of structured sparsity, N:M{\textcolor{blue}{Unify the N,M format in methods section with the previous sections.} sparsity is one of the most widely adopted patterns. In this scheme, for every group of M weights, only N are retained, and the remaining (M-N) are pruned. This structured pattern aligns well with modern hardware acceleration libraries, allowing for substantial speed-ups over unstructured sparsity, which is harder to exploit efficiently at the hardware level.

% Formally, for a weight tensor $W \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}} $, N:M sparsity enforces that each {\textcolor{red}{sub-vector with size M }contains exactly N non-zero elements, typically selected based on magnitude or importance criteria. While this improves inference efficiency, enforcing such structured patterns without significant accuracy drop remains a challenge.

% \noindent \textbf{Transformer Architectures.} Transformers have become the backbone of many state-of-the-art models in both vision and language domains. A standard Transformer block consists of a multi-head self-attention mechanism followed by a position-wise feed-forward network (FFN). The input to the model is a sequence of tokens $X \in \mathbb{R}^{N \times D}$, where $N$ is the number of tokens and $D$ is the feature dimension. The self-attention module enables tokens to attend to one another, capturing long-range dependencies, while the FFN transforms token features via two linear layers and a non-linear activation (\textit{e.g.}, GeLU). This structure is repeated across multiple layers, yielding deep and hierarchical feature representations.

% Due to the high dimensionality of intermediate activations and weights, Transformers present substantial opportunities for sparsification—especially in FFN layers and attention projections—while maintaining performance.

% \noindent \textbf{Permutation for Structural Sparsity.} {\textcolor{blue}{Permutation has been repeatedly introduced in introduction, related works, and here. Maybe you should have something new here, such as some detailed formula to avoid being considered as simply padding similar words. Also, adding some formula in 'structural sparsity' and 'Transformer Architecture' is better.} To better align model weights with structural sparsity patterns like N:M, permutation-based methods have recently gained attention. The core idea is to rearrange the rows or columns of weight matrices such that important weights are grouped together, making it easier to apply structured pruning without incurring significant information loss.

% For example, in channel permutation methods, the input or output channels of convolution or linear layers are reordered to maximize sparsity alignment, improving pruning effectiveness. Similarly, in Transformers, permutations can be applied to attention heads, hidden dimensions, or token positions to reorganize the model’s internal representation in a sparsity-friendly manner.

% However, most existing permutation strategies rely on hand-crafted heuristics or post-hoc optimization, which are non-differentiable and cannot be integrated into end-to-end training. This motivates the need for a learnable permutation framework, where permutations are jointly optimized with the network parameters using gradient-based methods. Such a framework can dynamically adapt to data and training objectives, yielding better sparsity patterns and minimal accuracy degradation.

\subsection{Our Learnable Permutator}
To enable structured pruning under the N:M sparsity constraint in transformer-based models, we propose a novel end-to-end learnable permutation framework.  Our method introduces a {\textcolor{blue}{No need to capitalize the first letter unless it is the start of the sentence or in the title.} Permutation Cost Predictor, a Bipartite Matching Solver, and a sparsity-aware training objective. Given the importance of element ordering in N:M sparsity — where each group of M elements must retain exactly N non-zero values — our framework learns a task-specific channel permutation that improves the alignment between model structure and pruning pattern.

Unlike existing heuristics (\textit{e.g.,} channel importance ranking), our method optimizes permutation globally and differentiably across all layers, leading to better compatibility with the structured sparsity mask. This is achieved by modeling permutation as a differentiable matching problem, {\textcolor{red}{training} with both cross-entropy supervision and layer-wise feature distillation.

\noident \textbf{Permutation Cost Predictor.}
The core of our method is a learnable Permutation Cost Predictor, which produces a cost matrix to guide the reordering of channels or features. For a given layer with weight matrix $W\in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$ 
, the goal is to learn a permutation matrix $ P \in \{0, 1\}^{d_{\text{in}} \times d_{\text{in}}}$
 that reorders input channels to better suit the N:M sparsity pattern. We define a cost matrix 
$
C \in \mathbb{R}^{d_{\text{in}} \times d_{\text{in}}}$, where 
$C_{i,j}$ quantifies the cost of mapping the original channel 
$i$ to position 
$j$. The cost matrix is parameterized by a light-weight neural predictor (\textit{e.g.,} MLP with positional encoding), and trained to reflect both pruning compatibility and semantic alignment. {\textcolor{blue}{Not clear for $C$. Is $C$ the input or output of the MLP? Does the MLP participate in the inference process of the original Transformer? What is the specific structure of the MLP?
Also, how does $P$ affect $W$? Use a formula such as $W'=P*W$ or something to connect them.}

\noident \textbf{Bipartite Matching Solver.}
To obtain the optimal permutation matrix 
{\textcolor{red}{$P^*$}}, we formulate the channel reordering problem as a bipartite matching task based on the cost matrix $C$. The objective is to solve:

\begin{equation}
{\textcolor{red}{P^*} = \arg\min_{P \in \mathcal{P}} \sum_{i=1}^{d_{\text{in}}} \sum_{j=1}^{d_{\text{in}}} P_{i,j} \cdot C_{i,j}
\end{equation}
where {\textcolor{blue}{$\mathcal P$?}$P$ denotes the set of valid permutation matrices (\textit{i.e.,} each row and column sums to 1).{\textcolor{blue}{Why sum to 1 be considered as a valid permutation matrix?} We use a differentiable matching solver (\textit{e.g.,} Gumbel-Sinkhorn [Mena et al.], SoftSort, or SparseSinkhorn) to allow gradient propagation through the discrete assignment process. The resulting soft permutation matrix is optionally binarized during inference to enable hardware-friendly structured sparsity.

\subsection{Optimization Losses}
To train the permutation framework in an end-to-end fashion, we introduce a joint loss function composed of:

\noident \textbf{End-to-End Cross-Entropy Loss.}
We apply standard task-specific loss (e.g., classification or language modeling cross-entropy) on the output of the pruned model, allowing the permutation and pruning to be optimized jointly with downstream objectives:
{\textcolor{blue}{What is the architecture of $f_{perm_prune}$? Not mentioned in previous.}
\begin{equation}
\mathcal{L}_{\text{task}} = \text{CE}(f_{\text{perm\_prune}}(x), y)
\end{equation}
\noident \textbf{Layer-wise Distillation Loss.}
To preserve the original feature representations despite pruning, we use a layer-wise distillation loss. Let $h_l ^{orig}
$ and $ h_l^{perm\_prune}$ {\textcolor{blue}{How do you get features after permutation pruning? No formula in previous.}
  denote the features of layer 
$l$ before and after permutation-pruning, we define:
\begin{equation}
    \mathcal{L}_{\text{distill}} = \sum_{l=1}^{L} \lambda_l \cdot \| h_l^{\text{orig}} - h_l^{\text{perm\_prune}} \|_2^2
\end{equation}

The final training objective is:
$\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \alpha \cdot \mathcal{L}_{\text{distill}}$, where $\alpha$ controls the distillation weight.

%\subsection{Training and Evaluation Process}


==> sections/methods_v2.tex <==
\section{Methods}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{Figures/perm_isbetter.pdf} 
\caption{The channel permutation process enhances the friendliness of the 2:4 sparsification, making the overall saliency of the pruning metric more preserved.}
\label{fig:channel-perm}
\end{figure}


In this section, we first introduce some preliminaries about channel permutation for N:M pruning Transformers. We then present our novel end-to-end learnable permutation framework, which incorporates a learnable permutation cost matrix, a differentiable bipartite matching solver, and a sparsity optimization loss function to directly optimize the permutation operator for both vision transformers and large language models.


\subsection{Preliminaries}
\label{sec:preliminaries}

\subsubsection{Channel Permutation for N:M Sparsity.} Channel permutation is an effective technique for enhancing the compatibility of neural network weights with structured sparsity patterns, such as 2:4 sparsity. As illustrated in Figure~\ref{fig:channel-perm}, the original weight layout may exhibit an uneven distribution of the saliency metric, where high or low values are concentrated within certain blocks. This non-uniformity poses challenges for fixed sparsity patterns to retain the most informative weights, often resulting in a lower overall saliency after pruning.

By applying channel permutation prior to pruning, saliency values can be redistributed more uniformly across blocks. This increases the likelihood that each 4-element group contains a representative mix of salient and non-salient weights, thereby improving the effectiveness of 2:4 sparsification. Consequently, more critical weights are preserved, leading to better retention of salient information in the pruned model.

\subsubsection{Channel Permutation for Linear Layers.} When applying a channel permutation to the input dimension of the weight matrix in a linear layer, it is essential to maintain output consistency by ensuring that the corresponding input activation is permuted in the same manner. Specifically, if a permutation matrix \( \mathbf{P} \) is applied to the input channels of the \( i \)-th layer’s weight matrix \( \mathbf{W}^{\top}_i  \in \mathbb{R}^{d_\text{in} \times d_\text{out}}\), i.e., \( \hat{\mathbf{W}}_{i}^{\top} = \mathbf{P} \mathbf{W}^{\top}_i\), then the input dimension of its activation \( \mathbf{A}_i \in \mathbb{R}^{d_\text{batch} \times d_\text{in}} \) must also be permuted as \( \hat{\mathbf{A}}_i = \mathbf{A}_i\mathbf{P}^{\top} \) to preserve the computation: \( \mathbf{\hat{A}}_{i+1} = \mathbf{\hat{A}}_{i}\mathbf{\hat{W}}^{\top}_{i+1} =\mathbf{A}_i\mathbf{P}^{\top}\mathbf{P} \mathbf{W}^{\top}_i  =\mathbf{A}_i \mathbf{W}^{\top}_i=\mathbf{A}_{i+1}\) ($\mathbf{P}^{\top} = \mathbf{P}^{-1}$). To avoid the computational cost of explicitly permuting activations at runtime, we can instead permute the output channels of the preceding \((i{-}1)\)-th layer’s weight matrix (\( \hat{\mathbf{W}}_{i-1} = \mathbf{W}_{i-1} \mathbf{P}^{\top} \)) to make \( \hat{\mathbf{A}}_{i} = \mathbf{A}_{i-1}\hat{\mathbf{W}}_{i-1} = \mathbf{A}_{i}\mathbf{P}^{\top}\), as shown in Figure~\ref{fig:perm_between_layers}. This strategy preserves functional equivalence while eliminating the need for activation reordering.


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm_between_layers.pdf} 
\caption{To guarantee output consistency, after the input channel of the $i$-th layer weight is permuted, the input activation of that layer should also be permuted accordingly, which can be realized by permuting the output channel of the previous $i-1$-th layer weight accordingly.}
\label{fig:perm_between_layers}
\end{figure}

\subsubsection{Channel Permutation for Transformers.} Transformer architecture goes far beyond sequential linear layers. As shown in Figure~\ref{fig:transformer_perm}, a typical Transformer block comprises two principal functional modules: a multi-head self-attention mechanism (MHA) and a feed-forward network (FFN). Given the incoming representation \( \mathbf{X}_{i-1} \) at layer \( i \), the transformed output \( \mathbf{X}_{i} \) is computed through this sequence of operations:

\begin{equation}
\label{eq:1}
\begin{aligned}
    \mathbf{A} &= \text{LayerNorm}\left(\mathbf{A}_{i-1} + \operatorname{MHA}(\mathbf{A}_{i-1})\right), \\
    \mathbf{A}_i &= \text{LayerNorm}\left(\mathbf{A} + \mathrm{FFN}(\mathbf{A})\right).
\end{aligned}
\end{equation}

In the multi-head self-attention (MHA) module, the projection matrices \( \mathbf{W}_q \), \( \mathbf{W}_k \), and \( \mathbf{W}_v \) map the same input into query, key, and value representations, respectively, and thus share a common input channel structure. To maintain their functional alignment, any channel permutation must be applied jointly to all three matrices. Moreover, when doing input channel permutation for the mapping weight $\mathbf{W}_o$ for attention output, \( \mathbf{W}_q \), \( \mathbf{W}_k \), and \( \mathbf{W}_v \) should also do the corresponding output channel permutation in an aggregated manner. The feed-forward network (FFN) follows a similar structure: \( \mathbf{W}_{up} \) and \( \mathbf{W}_{gate} \) operate on the same input and must share the same permutation, while their output permutation must align with the input of the down-projection matrix \( \mathbf{W}_{down} \). Therefore, channel permutation must be designed and applied in a structured, group-wise manner to preserve the internal consistency of MHA and FFN submodules. 
% A detailed theoretical justification for these constraints is provided in Appendix~X.


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/transformer_perm.pdf} 
\caption{An overview of channel permutation for Transformer layers. $W_q$, $W_k$, and $W_v$ need to learn their input channel permutation in an aggregated way and make corresponding adjustments in their output channel for $W_o$'s input channel permutation. $W_{gate}$ and $W_{up}$ are congruent.}
\label{fig:transformer_perm}
\end{figure}

% \noindent \textbf{Structural Sparsity.} Structural sparsity has emerged as a promising approach to reduce the computational and memory overhead of deep neural networks while retaining hardware efficiency. Among various forms of structured sparsity, N:M{\textcolor{blue}{Unify the N,M format in methods section with the previous sections.} sparsity is one of the most widely adopted patterns. In this scheme, for every group of M weights, only N are retained, and the remaining (M-N) are pruned. This structured pattern aligns well with modern hardware acceleration libraries, allowing for substantial speed-ups over unstructured sparsity, which is harder to exploit efficiently at the hardware level.

% Formally, for a weight tensor $W \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}} $, N:M sparsity enforces that each {\textcolor{red}{sub-vector with size M }contains exactly N non-zero elements, typically selected based on magnitude or importance criteria. While this improves inference efficiency, enforcing such structured patterns without significant accuracy drop remains a challenge.

% \noindent \textbf{Transformer Architectures.} Transformers have become the backbone of many state-of-the-art models in both vision and language domains. A standard Transformer block consists of a multi-head self-attention mechanism followed by a position-wise feed-forward network (FFN). The input to the model is a sequence of tokens $X \in \mathbb{R}^{N \times D}$, where $N$ is the number of tokens and $D$ is the feature dimension. The self-attention module enables tokens to attend to one another, capturing long-range dependencies, while the FFN transforms token features via two linear layers and a non-linear activation (\textit{e.g.}, GeLU). This structure is repeated across multiple layers, yielding deep and hierarchical feature representations.

% Due to the high dimensionality of intermediate activations and weights, Transformers present substantial opportunities for sparsification—especially in FFN layers and attention projections—while maintaining performance.

% \noindent \textbf{Permutation for Structural Sparsity.} {\textcolor{blue}{Permutation has been repeatedly introduced in introduction, related works, and here. Maybe you should have something new here, such as some detailed formula to avoid being considered as simply padding similar words. Also, adding some formula in 'structural sparsity' and 'Transformer Architecture' is better.} To better align model weights with structural sparsity patterns like N:M, permutation-based methods have recently gained attention. The core idea is to rearrange the rows or columns of weight matrices such that important weights are grouped together, making it easier to apply structured pruning without incurring significant information loss.

% For example, in channel permutation methods, the input or output channels of convolution or linear layers are reordered to maximize sparsity alignment, improving pruning effectiveness. Similarly, in Transformers, permutations can be applied to attention heads, hidden dimensions, or token positions to reorganize the model’s internal representation in a sparsity-friendly manner.

% However, most existing permutation strategies rely on hand-crafted heuristics or post-hoc optimization, which are non-differentiable and cannot be integrated into end-to-end training. This motivates the need for a learnable permutation framework, where permutations are jointly optimized with the network parameters using gradient-based methods. Such a framework can dynamically adapt to data and training objectives, yielding better sparsity patterns and minimal accuracy degradation.

\subsection{Our Learnable Permutator}
To enable structured pruning under the N:M sparsity constraint in transformer-based models, we propose a novel end-to-end learnable permutation framework.  Our method introduces a permutation cost predictor, a bipartite matching solver, and a sparsity-aware training objective. Given the importance of element ordering in N:M sparsity, our framework learns a task-specific channel permutation that improves the alignment between model structure and pruning pattern.

Unlike existing heuristics (\textit{e.g.,} channel importance ranking), our method optimizes permutation globally and differentiably across all layers, leading to better compatibility with the structured sparsity mask. This is achieved by modeling permutation as a differentiable matching problem, optimizing the cost predictor with both cross-entropy supervision and layer-wise feature distillation.
\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{LaTeX/Figures/overview.pdf} 
\vspace{-4mm}
\caption{Overview of our learnable permutation. Our method introduces a learnable permutation cost predictor to generate cost matrices for the linear layers in a Transformer model. These cost matrices are used to obtain optimal permutation matrices via a bipartite matching solver. The layer weights are then permuted by multiplying them with the corresponding permutation matrices.
Next, a mask generator identifies the less important weights using the N:M semi-structured pruning scheme, producing N:M sparsity masks. These masks are then transformed into permuted masks by applying the inverse of the previously computed permutation matrices.
Finally, the permuted masks are applied to the corresponding layer weights, and the resulting masked weights are used in the layer computations in place of the original weights. To enable gradient flow through the binary
masks, we apply Straight-Through Estimation (STE) and train our model using our sparsity optimization loss.}
\label{fig:overview}
\end{figure*}

\subsubsection{Permutation Cost Predictor.}
The core of our method is a learnable permutation cost predictor, which produces a cost matrix to guide the reordering of channels or features. For a given layer with weight matrix $W\in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$ 
, the goal is to learn a permutation matrix $ P \in \{0, 1\}^{d_{\text{in}} \times d_{\text{in}}}$
 that reorders input channels to better suit the N:M sparsity pattern. We define a cost matrix 
$
C \in \mathbb{R}^{d_{\text{in}} \times d_{\text{in}}}$, where 
$C_{i,j}$ quantifies the cost of mapping the original channel 
$i$ to position 
$j$. The cost matrix is parameterized by a light-weight neural predictor (\textit{e.g.,} MLP with positional encoding), and trained to reflect both pruning compatibility and semantic alignment. %{\textcolor{blue}{Not clear for $C$. Is $C$ the input or output of the MLP? Does the MLP participate in the inference process of the original Transformer? What is the specific structure of the MLP?
%Also, how does $P$ affect $W$? Use a formula such as $W'=P*W$ or something to connect them.}

% \noident \textbf{Bipartite Matching Solver.}
% To obtain the optimal permutation matrix 
% $P^*$, we formulate the channel reordering problem as a bipartite matching task based on the cost matrix $C$. The objective is to solve:

% \begin{equation}
% {P^* = \arg\min_{P \in \mathcal{P}} \sum_{i=1}^{d_{\text{in}}} \sum_{j=1}^{d_{\text{in}}} P_{i,j} \cdot C_{i,j}
% \end{equation}
% where $\mathcal P$ denotes the set of valid permutation matrices (\textit{i.e.,} each row and column sums to 1). We use a differentiable matching solver (\textit{e.g.,} Gumbel-Sinkhorn [Mena et al.], SoftSort, or SparseSinkhorn) to allow gradient propagation through the discrete assignment process. The resulting soft permutation matrix is optionally binarized during inference to enable hardware-friendly structured sparsity.

\subsubsection{Differentiable Biparate Matching Solver.}
We cast channel reordering within each group of size $N$ as a bipartite matching with cost matrix $C\in\mathbb{R}^{N\times N}$. The discrete problem $\min_{P\in\mathcal{P}}\langle C,P\rangle$, where $\mathcal{P}$ is the set of permutation matrices, is relaxed to the Birkhoff polytope
\[
\mathcal{B}_N=\{P\ge 0:\; P\mathbf{1}=\mathbf{1},\; P^{\top}\mathbf{1}=\mathbf{1}\}.
\]
We solve the entropic optimal transport objective
\[
\min_{P\in\mathcal{B}_N}\;\langle C,P\rangle+\varepsilon\sum_{i,j} P_{ij}(\log P_{ij}-1),
\]
whose KKT conditions imply $P=\mathrm{Diag}(u)\,K\,\mathrm{Diag}(v)$ with $K=\exp(-C/\varepsilon)$. The unknown scalings are obtained by iterative proportional fitting in the log domain
\[
\log u \leftarrow -\,\mathrm{logsumexp}(\log K+\log v,\,1),
\]
\[
\log v \leftarrow -\,\mathrm{logsumexp}(\log K^{\top}+\log u,\,1),
\]
which enforces unit row and column sums. A decreasing temperature schedule $\varepsilon_t$ sharpens $P$ toward an extreme point, yielding a nearly binary assignment while keeping the mapping differentiable. The soft permutation is applied blockwise to weights, for example $W' = P W$, so gradients propagate through the normalization steps into the cost network and the permutator.

At inference, we discretize by solving the linear assignment
\[
\Pi=\arg\min_{P\in\mathcal{P}}\langle C,P\rangle,
\]
using the Hungarian algorithm, which returns a one to one mapping in $O(N^{3})$ time per group and produces a hardware friendly structured permutation. The training cost per group is $O(N^{2}T)$ in time and $O(N^{2})$ in memory, hence the total cost grows linearly with the number of groups and quadratically with the group size. This interface also supports Gumbel Sinkhorn for exploration, SoftSort for rank based costs, and SparseSinkhorn for sharper doubly stochastic solutions.



\subsection{Optimization Losses}
To train the permutation framework in an end-to-end fashion, we introduce a joint loss function composed of:

\subsubsection{End-to-End Cross-Entropy Loss.}
We apply standard task-specific loss (e.g., classification or language modeling cross-entropy) on the output of the pruned model, allowing the permutation and pruning to be optimized jointly with downstream objectives:
\begin{equation}
\mathcal{L}_{\text{task}} = \text{CE}(f_{\text{perm\_prune}}(x), y)
\end{equation} 
where $f_{\text{perm\_prune}}$
denotes the application of permutation followed by N:M semi-structured pruning on the original Transformer model.

\subsubsection{Layer-wise Distillation Loss.}
To preserve the original feature representations despite pruning, we use a layer-wise distillation loss. 
Given the same input to layer $l$, let 
$h_l ^{orig}
$ and $ h_l^{perm\_prune}$
represent the output features of the layer without and with permutation-pruning, respectively.
we define:
\begin{equation}
    \mathcal{L}_{\text{distill}} = \sum_{l=1}^{L} \lambda_l \cdot \| h_l^{\text{orig}} - h_l^{\text{perm\_prune}} \|_2^2
\end{equation}
where $L$ denotes the number of pruning layers and $\lambda_l$ denotes the loss weight of layer $l$.

The final training objective is:
$\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \alpha \cdot \mathcal{L}_{\text{distill}}$, where $\alpha$ controls the distillation weight.

%\subsection{Training and Evaluation Process}
\subsection{Training and Inference Details}

During training, we first run the original Transformer model for several hundred forward passes to collect the running mean of input features at each layer. This accumulated feature statistics are used to guide the semi-structured pruning process performed by the mask generator.
Next, we freeze all weights of the Transformer model and enable updates only for the parameters of the permutation cost predictor. To handle alignment issues among the Q, K, and V projections in attention layers, we adopt a grouped permutation strategy. The permutation cost predictor is then optimized using our proposed sparsity optimization loss.

During inference, the permutation cost predictor is frozen. We employ a bipartite matching solver to compute the optimal permutation matrices for each layer. The layer weights are combined with the sparsity masks produced by the mask generator to perform N:M semi-structured pruning on the original Transformer. The pruned model is then used for standard Transformer inference.






==> sections/methods_v3.tex <==
\section{Methods}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{Figures/perm_isbetter.pdf} 
\caption{The channel permutation process enhances the friendliness of the 2:4 sparsification, making the overall saliency of the pruning metric more preserved.}
\label{fig:channel-perm}
\end{figure}


We begin by introducing preliminaries on channel permutation in the context of optimizing structured N:M sparsity for Transformers. We then describe our proposed end-to-end learnable permutation framework, which consists of a learnable cost prediction module, a differentiable bipartite matching solver, and sparsity-aware optimization objectives. This unified design enables direct optimization of permutation operators for both vision transformers, large language models, and vision-language models.


\subsection{Preliminaries}
\label{sec:preliminaries}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm_between_layers.pdf} 
\caption{Channel permutation for Linear layers. To guarantee output consistency, after the input channel of the $i$-th layer weight is permuted, the input activation of that layer should also be permuted accordingly, which can be realized by permuting the output channel of the previous ($i-1$)-th layer weight accordingly.}
\label{fig:perm_between_layers}
\end{figure}

\subsubsection{Optimize N:M Sparsity via Channel Permutation.} 
Channel permutation improves the compatibility of weight tensors with structured sparsity patterns such as N:M sparsity. As shown in Figure~\ref{fig:channel-perm}, the original layout may exhibit an imbalanced distribution of saliency, where highly salient weights are concentrated within certain groups. This local skewness reduces the likelihood that fixed sparsity patterns retain important weights, often leading to suboptimal pruning results with low total preserved saliency.
By permuting channels before pruning, the saliency metric is redistributed more evenly across groups. This increases the probability that each M-element group includes a mix of salient and non-salient weights, enabling the structured sparsification process to preserve more informative elements. As a result, channel permutation improves the effectiveness of N:M pruning by aligning the weight layout with the constraints of structured sparsity.

To effectively apply channel permutation for structured sparsity, it is essential to consider how permutation interacts with the computational graph of the model. In practice, modern architectures consist of a variety of structural units, ranging from simple linear layers to highly interdependent Transformer blocks. We therefore analyze channel permutation in two representative settings: linear layers, where permutation can be propagated analytically between adjacent layers, and Transformer blocks, which require more careful coordination due to shared and coupled weight structures across multiple projections.


\subsubsection{Channel Permutation for Linear Layers.} 
When applying a channel permutation to the input dimension of a linear layer, it is necessary to preserve output consistency by maintaining alignment between the permuted weight matrix and its corresponding input activation. Let \(\mathbf{W}_i^{\top} \in \mathbb{R}^{d_\text{in} \times d_\text{out}}\) be the weight matrix of the \(i\)-th linear layer, and let \(\mathbf{P}\in\mathbb{R}^{d_\text{in} \times d_\text{in}}\) be a permutation matrix. Applying the permutation to the input channels of the weight yields \(\widehat{\mathbf{W}}_i^{\top} = \mathbf{P} \mathbf{W}_i^{\top}\). To maintain correct computation, the corresponding activation \(\mathbf{A}_i \in \mathbb{R}^{d_\text{batch} \times d_\text{in}}\) must also be transformed as \(\widehat{\mathbf{A}}_i = \mathbf{A}_i \mathbf{P}^{\top}\), so that the output remains unchanged:
\[
\widehat{\mathbf{A}}_{i+1} = \widehat{\mathbf{A}}_i \widehat{\mathbf{W}}_i^{\top} = \mathbf{A}_i \mathbf{P}^{\top} \mathbf{P} \mathbf{W}_i^{\top} = \mathbf{A}_i \mathbf{W}_i^{\top} = \mathbf{A}_{i+1},
\]
where the last equality holds since \(\mathbf{P}^{\top} = \mathbf{P}^{-1}\).

To avoid runtime activation permutation, we propagate the permutation backward to the output channels of the preceding \((i{-}1)\)-th layer. Specifically, we set \(\widehat{\mathbf{W}}_{i-1} = \mathbf{W}_{i-1} \mathbf{P}^{\top}\), so that
\[
\widehat{\mathbf{A}}_i = \mathbf{A}_{i-1} \widehat{\mathbf{W}}_{i-1} = \mathbf{A}_{i-1} \mathbf{W}_{i-1} \mathbf{P}^{\top} = \mathbf{A}_i \mathbf{P}^{\top}.
\]
This transformation ensures functional equivalence without requiring explicit reordering of activations at runtime, as illustrated in Figure~\ref{fig:perm_between_layers}.


\subsubsection{Channel Permutation for Transformer Layers.} 
Applying channel permutation in Transformer architectures presents unique challenges due to the complex structural coupling within multi-head self-attention (MHA) and feed-forward network (FFN) submodules. Unlike sequential linear layers, Transformer blocks involve parallel projections that share input representations and interdependent weight matrices, requiring permutation to be applied in a coordinated and structure-aware manner, as shown in Figure~\ref{fig:transformer_perm}.

In the MHA module, the input \(\mathbf{X}\in\mathbb{R}^{B\times T\times d_{\text{hidden}}}\) is projected into query, key, and value tensors using three parameter matrices \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) for attention computation and generate \( \mathbf{X}_\text{Attn} \in \mathbb{R}^{B\times T\times d_{\text{hidden}}} \), which will be projected into \(\mathbf{W}^{\top}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\). Since \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v}\) operates on the same input, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{hidden}}\times d_{\text{hidden}}}\) for \( \mathbf{W}^{\top}_\mathrm{o} \) should be applied identically to the others' output channels:

\[
\begin{aligned}
\widehat{\mathbf{W}}^{\top}_\mathrm{q} = \mathbf{W}^{\top}_\mathrm{q} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{k} = \mathbf{W}^{\top}_\mathrm{k} \mathbf{P}^{\top}_{\text{in}}, \\
\widehat{\mathbf{W}}^{\top}_\mathrm{v} = \mathbf{W}^{\top}_\mathrm{v} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{o} = \mathbf{P}_{\text{in}} \mathbf{W}^{\top}_\mathrm{o}.
\end{aligned}
\]


% To maintain downstream consistency, the corresponding output projection matrix \(\mathbf{W}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) must absorb the inverse permutation on its input channels:
% $\mathbf{W}_o^{\prime} = \mathbf{W}_o \mathbf{P}_{\text{in}}^{\top}$.


Similarly, the permutation of the input channel for \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \) requires implementation of the corresponding output channel permutation for the previous layer. The FFN submodule typically consists of two parallel expansion matrices \(\mathbf{W}^{\top}_{\mathrm{up}}, \mathbf{W}^{\top}_{\mathrm{gate}} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{ff}}}\) followed by a down-projection \(\mathbf{W}^{\top}_{\mathrm{down}} \in \mathbb{R}^{d_{\text{ff}} \times d_{\text{hidden}}}\). The two expansion paths operate on the same input and their outputs are combined multiplicatively. Therefore, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{ff}}\times d_{\text{ff}}}\) for \( \mathbf{W}^{\top}_\mathrm{down} \) should be applied identically to the others' output channels:

{\small
\[
\widehat{\mathbf{W}}_{\mathrm{up}} =  \mathbf{W}^{\top}_{\mathrm{up}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{gate}} =  \mathbf{W}^{\top}_{\mathrm{gate}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{down}} =  \mathbf{P}_{\text{in}}\mathbf{W}^{\top}_{\mathrm{down}}.
\]
}


These constraints highlight the key challenge: channel permutation in Transformers cannot be applied independently to each weight matrix, but must instead follow structured, bounded rules that preserve functional dependencies within each block. As such, we design our permutation system to operate jointly over bounded parameters, enforcing permutation sharing and inverse propagation where required. This ensures that permutation-aware sparsification maintains semantic alignment and preserves compatibility with structured weight compression.


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/transformer_perm.pdf} 
\caption{An overview of channel permutation for Transformer layers. $\mathbf{W}_\mathrm{q}$, $\mathbf{W}_\mathrm{k}$, and $\mathbf{W}_\mathrm{v}$ need to learn their input channel permutation in an aggregated way and make corresponding adjustments in their output channel for $\mathbf{W}_\mathrm{o}$'s input channel permutation. $\mathbf{W}_\mathrm{gate}$ and $\mathbf{W}_\mathrm{up}$ are congruent.}
\label{fig:transformer_perm}
\end{figure}



\subsection{Learnable Channel Permutator}
\label{sec:perm}

To support structured pruning under the N:M sparsity constraint in Transformer-based architectures, we introduce a learnable channel permutation framework that enables end-to-end optimization of permutation operators. The core idea is to adaptively reorder the input and output channels of weight matrices such that the resulting structure is more compatible with fixed pruning patterns. This is especially critical in N:M sparsity, where preserving the most informative weights within each group requires aligning saliency patterns with the imposed structure.

Our framework consists of three components: a permutation cost predictor, a differentiable bipartite matching solver, and a sparsity-aware training objective. Unlike prior heuristics that rely on local importance scores or static channel ranking, our method learns permutation jointly and differentiably across layers. By modeling the permutation process as a differentiable matching problem, we enable global coordination and gradient-based optimization. The cost predictor is trained with supervision from both final-task cross-entropy loss and intermediate layer-wise feature distillation, allowing the learned permutation to capture both global semantic alignment and structural sparsity compatibility.

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{LaTeX/Figures/overview_new.pdf} 
\vspace{-4mm}
\caption{Overview of our learnable permutation. Our method introduces a learnable permutation cost predictor to generate cost matrices for the linear layers in a Transformer model. These cost matrices are used to obtain optimal permutation matrices via a bipartite matching solver. The layer weights are then permuted by multiplying them with the corresponding permutation matrices.
Next, a mask generator identifies the less important weights using the N:M semi-structured pruning scheme, producing N:M sparsity masks. These masks are then transformed into permuted masks by applying the inverse of the previously computed permutation matrices.
Finally, the permuted masks are applied to the corresponding layer weights, and the resulting masked weights are used in the layer computations in place of the original weights. To enable gradient flow through the binary
masks, we apply Straight-Through Estimation (STE) and train our model using our sparsity optimization loss.}
\label{fig:overview}
\end{figure*}

\subsubsection{Permutation Cost Predictor.}
\label{sec:cost}
The core of our method is a learnable permutation cost predictor, which produces a cost matrix to guide the reordering of channels or features. 
Given a weight matrix \(\mathbf{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}\) from a weight matrix, the goal is to construct a permutation matrix \(\mathbf{P} \in \{0,1\}^{d_{\text{in}} \times d_{\text{in}}}\) that rearranges the input channels such that the pruned model aligns more effectively with structured N:M sparsity constraints.

To enable differentiable learning of \(\mathbf{P}\), we introduce a real-valued cost matrix \(\mathbf{C} \in \mathbb{R}^{d_{\text{in}} \times d_{\text{in}}}\), where each element \(C_{i,j}\) reflects the cost of assigning the original input channel \(i\) to position \(j\). Intuitively, \(\mathbf{C}\) encodes the pairwise preference for spatial relocation, integrating both structural sparsity alignment and semantic preservation objectives.
We parameterize the cost matrix using a lightweight neural network. For each input channel, we extract a feature vector \(f_i\) that summarizes the channel’s statistical or semantic properties, such as magnitude, variance, or learned embeddings. These features are first augmented with relative positional encodings to encode target indices \(j\), then passed through a  MLP layer \(h_\theta\) to produce the score:
\[
C_{i,j} = h_\theta\big(\text{concat}(f_i, \mathrm{PE}(j))\big),
\]
where \(\mathrm{PE}(j)\) denotes the positional encoding of index \(j\). This formulation allows the predictor to model both channel-wise importance and positional compatibility jointly. The resulting cost matrix serves as the input to the differentiable matching solver.



%{\textcolor{blue}{Not clear for $C$. Is $C$ the input or output of the MLP? Does the MLP participate in the inference process of the original Transformer? What is the specific structure of the MLP?
%Also, how does $P$ affect $W$? Use a formula such as $W'=P*W$ or something to connect them.}

% \noident \textbf{Bipartite Matching Solver.}
% To obtain the optimal permutation matrix 
% $P^*$, we formulate the channel reordering problem as a bipartite matching task based on the cost matrix $C$. The objective is to solve:

% \begin{equation}
% {P^* = \arg\min_{P \in \mathcal{P}} \sum_{i=1}^{d_{\text{in}}} \sum_{j=1}^{d_{\text{in}}} P_{i,j} \cdot C_{i,j}
% \end{equation}
% where $\mathcal P$ denotes the set of valid permutation matrices (\textit{i.e.,} each row and column sums to 1). We use a differentiable matching solver (\textit{e.g.,} Gumbel-Sinkhorn [Mena et al.], SoftSort, or SparseSinkhorn) to allow gradient propagation through the discrete assignment process. The resulting soft permutation matrix is optionally binarized during inference to enable hardware-friendly structured sparsity.

\subsubsection{Differentiable Bipartite Matching Solver.}
\label{sec:match}

Directly learning full permutation matrices for large-dimensional weight tensors in Transformer models is computationally expensive and often unnecessary. To improve scalability and reduce overhead, we adopt a group-wise permutation strategy, where the input channels of each layer are partitioned into non-overlapping groups of fixed size \(N\), and a separate permutation is learned within each group. This design not only reduces the number of parameters in the permutation predictor and solver, but also aligns naturally with hardware-efficient structured pruning, where pruning is applied in fixed-size blocks.

Formally, given a predicted cost matrix \(\mathbf{C} \in \mathbb{R}^{N \times N}\) for a single group, we frame channel permutation as a bipartite matching problem. The objective is to find a permutation matrix \(\mathbf{P} \in \mathcal{P}\), where \(\mathcal{P}\) denotes the set of \(N \times N\) permutation matrices, that minimizes the total matching cost:
\[
\min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle.
\]
However, this combinatorial optimization is non-differentiable and incompatible with gradient-based training. To enable end-to-end learning, we adopt a continuous relaxation by replacing \(\mathcal{P}\) with the Birkhoff polytope \(\mathcal{B}_N\), the convex hull of all permutation matrices:
\[
\mathcal{B}_N = \left\{ \mathbf{P} \in \mathbb{R}^{N \times N} \,\middle|\, \mathbf{P} \ge 0,\; \mathbf{P} \mathbf{1} = \mathbf{1},\; \mathbf{P}^{\top} \mathbf{1} = \mathbf{1} \right\}.
\]

We then solve the entropy-regularized optimal transport problem:
\[
\min_{\mathbf{P} \in \mathcal{B}_N} \langle \mathbf{C}, \mathbf{P} \rangle + \varepsilon \sum_{i,j} P_{ij} (\log P_{ij} - 1),
\]
which admits a solution of the form \(\mathbf{P} = \mathrm{Diag}(u)\, \mathbf{K} \, \mathrm{Diag}(v)\), where \(\mathbf{K} = \exp(-\mathbf{C} / \varepsilon)\). The scaling vectors \(u\) and \(v\) are computed via Sinkhorn iterations in the log domain:
\[
\log u \leftarrow -\,\mathrm{logsumexp}(\log \mathbf{K} + \log v,\; \text{dim}=1),
\]
\[
\log v \leftarrow -\,\mathrm{logsumexp}(\log \mathbf{K}^{\top} + \log u,\; \text{dim}=1).
\]
This iterative process enforces doubly stochastic constraints while maintaining numerical stability. We anneal the temperature \(\varepsilon_t\) over iterations, which progressively sharpens the soft assignment \(\mathbf{P}\) toward a discrete permutation while preserving differentiability. The resulting \(\mathbf{P}\) is applied blockwise to reorder channels, e.g., \(\mathbf{W}' = \mathbf{P} \mathbf{W}\), allowing gradients to flow through the solver back into the cost predictor and upstream network.

At inference, we convert \(\mathbf{P}\) into a discrete permutation by solving the original assignment problem:
\[
\Pi = \arg\min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle,
\]
using the Hungarian algorithm, which yields an exact one-to-one mapping in \(O(N^3)\) time per group. This produces a hardware-efficient permutation suitable for structured sparse deployment.

The solver’s time and space complexity scale as \(O(N^2 T)\) and \(O(N^2)\) per group, respectively, where \(T\) is the number of Sinkhorn iterations. Since the procedure is applied independently to each group, the overall cost grows linearly with the number of groups and quadratically with group size, consistent with our scalability results.

In addition to the Sinkhorn-based solver, our framework supports alternative differentiable relaxations, including Gumbel-Sinkhorn for stochastic exploration, SoftSort for rank-sensitive objectives, and SparseSinkhorn for promoting sharper sparsity in the doubly stochastic matrix.




\subsection{End-to-End Optimization Objectives}
\label{sec:loss}

To enable joint learning of channel permutation and structured pruning, we train the framework using a composite loss function that integrates both task-level supervision and intermediate feature alignment. This promotes not only the retention of end-task performance but also structural consistency within the model.

\subsubsection{Task-Level Cross-Entropy Loss}
We apply a standard cross-entropy loss to the output of the pruned model, allowing the permutation parameters to be optimized directly for task performance. Let \(f_{\text{perm+prune}}(x)\) denote the output of the model after applying learned permutation followed by N:M structured pruning. The task loss is defined as:
\[
\mathcal{L}_{\text{task}} = \mathrm{CE}(f_{\text{perm+prune}}(x),\, y),
\]
where \(\mathrm{CE}(\cdot)\) is the cross-entropy loss and \(y\) is the ground-truth label. This loss ensures that the permutation contributes to preserving the discriminative capacity of the network.

\subsubsection{Layer-Wise Distillation Loss}
To preserve internal feature semantics despite pruning and permutation, we incorporate a layer-wise distillation loss that aligns intermediate representations between the original and the permuted-pruned models. Let \(h_l^{\text{orig}}\) and \(h_l^{\text{perm+prune}}\) denote the output features of the \(l\)-th layer in the original and permuted-pruned models, respectively. The distillation loss is defined as:
\[
\mathcal{L}_{\text{distill}} = \sum_{l=1}^{L} \lambda_l \, \| h_l^{\text{orig}} - h_l^{\text{perm+prune}} \|_2^2,
\]
where \(L\) is the number of pruned layers and \(\lambda_l\) is a layer-specific weighting factor. This objective encourages the permutator to preserve task-relevant internal representations, improving compatibility with the original model behavior.

\subsubsection{Final Objective}
The total loss is a weighted combination of task-level and distillation objectives:
\[
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \alpha \, \mathcal{L}_{\text{distill}},
\]
where \(\alpha\) is a hyperparameter controlling the influence of intermediate feature alignment. This joint objective provides both global task supervision and local structural guidance for effective permutation learning.


%\subsection{Training and Evaluation Process}
\subsection{Training and Inference Details}

\paragraph{Training.}  
We begin by collecting input feature statistics for each layer of the pretrained Transformer. Specifically, we perform several hundred forward passes to accumulate running estimates of activation means, which are later used by the sparsity mask generator to guide semi-structured pruning decisions. After this preprocessing stage, all Transformer weights are frozen, and only the parameters of the permutation cost predictor remain trainable.

To preserve structural consistency in attention layers, we impose a synchronized permutation constraint across coupled projection matrices, such as \(\mathbf{W}_q\), \(\mathbf{W}_k\), and \(\mathbf{W}_v\). These matrices share the same input representation, and applying inconsistent permutations would disrupt their joint computation. Prior heuristic permutation methods often ignore this constraint, resulting in mismatched projections that undermine both model functionality and compatibility with hardware-efficient execution. By enforcing a shared permutation across structurally dependent components, our method ensures correctness and preserves the potential for real-world acceleration under structured sparsity.


\paragraph{Inference.}  
At inference time, the learned permutation cost predictor is frozen. For each group of channels, we compute the optimal permutation matrix by solving the bipartite matching problem described in Section~\ref{sec:match}. These permutations are applied to reorder the weights of each layer, followed by the application of N:M sparsity masks generated from the collected feature statistics. The resulting pruned model, with permuted and sparsified weights, is then used for standard Transformer inference.







==> sections/methods_v4.tex <==
\section{Methods}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{Figures/perm_isbetter.pdf} 
\caption{The channel permutation process enhances the friendliness of the 2:4 sparsification, making the overall saliency of the pruning metric more preserved.}
\label{fig:channel-perm}
\vspace{-4mm}
\end{figure}


We begin by introducing preliminaries on channel permutation in the context of optimizing structured N:M sparsity for Transformers. We then describe our proposed end-to-end learnable permutation framework, which consists of a learnable cost prediction module, a differentiable bipartite matching solver, and  optimization objectives. 
The unified framework facilitates end-to-end optimization of permutation operators for diverse transformer-based architectures, including vision, language, and vision-language models.



\subsection{Preliminaries}
\label{sec:preliminaries}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm_between_layers.pdf} 
\caption{Channel permutation for Linear layers. To guarantee output consistency, after the input channel of the $i$-th layer weight is permuted, the input activation of that layer should also be permuted accordingly, which can be realized by permuting the output channel of the previous ($i-1$)-th layer weight accordingly.}
\label{fig:perm_between_layers}
\vspace{-4mm}
\end{figure}

\paragraph{Optimize N:M Sparsity via Channel Permutation.} 
Channel permutation enhances the compatibility of weight tensors with structured sparsity patterns such as N:M sparsity. As shown in Figure~\ref{fig:channel-perm}, the weight layout often exhibits uneven saliency, with important weights clustered within certain groups. This skewed distribution lowers the chance of retaining key weights under fixed 2:4 sparsity, resulting in suboptimal pruning with reduced preserved saliency.

By permuting channels before pruning, saliency becomes more evenly distributed across groups. This increases the likelihood that each M-element group contains a mix of important and unimportant weights, allowing structured pruning to retain more informative elements. Channel permutation thus improves N:M pruning by aligning weight layout with sparsity constraints.

% To effectively apply channel permutation for structured sparsity, it is essential to consider how permutation interacts with the computational graph of the model. In practice, modern architectures consist of a variety of structural units, ranging from simple linear layers to highly interdependent Transformer blocks. We therefore analyze channel permutation in two representative settings: linear layers, where permutation can be propagated analytically between adjacent layers, and Transformer blocks, which require more careful coordination due to shared and coupled weight structures across multiple projections.


\paragraph{Channel Permutation for Linear Layers.} 
Applying a channel permutation to a linear layer's input dimension requires aligning the permuted weights with its input activation to preserve output consistency. Let \(\mathbf{W}_i^{\top} \in \mathbb{R}^{d_\text{in} \times d_\text{out}}\) be the weight matrix of the \(i\)-th linear layer, and let \(\mathbf{P}\in \{0,1\}^{d_\text{in} \times d_\text{in}}\) be a permutation matrix. Applying input channel permutation to the weight yields \(\widehat{\mathbf{W}}_i^{\top} = \mathbf{P} \mathbf{W}_i^{\top}\). To maintain correct computation, the corresponding activation \(\mathbf{A}_i \in \mathbb{R}^{d_\text{batch} \times d_\text{in}}\) must also be transformed as \(\widehat{\mathbf{A}}_i = \mathbf{A}_i \mathbf{P}^{\top}\), so that the output remains unchanged (\(\mathbf{P}^{\top} = \mathbf{P}^{-1}\)):

\begin{equation}
   \widehat{\mathbf{A}}_{i+1} = \widehat{\mathbf{A}}_i \widehat{\mathbf{W}}_i^{\top} = \mathbf{A}_i \mathbf{P}^{\top} \mathbf{P} \mathbf{W}_i^{\top} = \mathbf{A}_i \mathbf{W}_i^{\top} = \mathbf{A}_{i+1}, 
   \label{eq:1}
\end{equation}

% where the last equality holds since .

To avoid runtime activation permutation, we propagate the permutation backward to the output channels of the preceding \((i{-}1)\)-th layer (\(\widehat{\mathbf{W}}_{i-1} = \mathbf{W}_{i-1} \mathbf{P}^{\top}\)), as shown in Figure~\ref{fig:perm_between_layers}, so that

\begin{equation}
    \widehat{\mathbf{A}}_i = \mathbf{A}_{i-1} \widehat{\mathbf{W}}_{i-1} = \mathbf{A}_{i-1} \mathbf{W}_{i-1} \mathbf{P}^{\top} = \mathbf{A}_i \mathbf{P}^{\top}.
    \label{eq:2}
\end{equation}

% This transformation ensures functional equivalence without requiring explicit reordering of activations at runtime, as illustrated in Figure~\ref{fig:perm_between_layers}.


\paragraph{Channel Permutation for Transformer Layers.} 
Applying channel permutation in Transformer architectures presents unique challenges due to the complex structural coupling within multi-head self-attention (MHA) and feed-forward network (FFN) submodules. Unlike sequential linear layers, Transformer blocks involve parallel projections that share input representations and interdependent weight matrices, requiring permutation to be applied in a coordinated and structure-aware manner, as shown in Figure~\ref{fig:transformer_perm}.

In the MHA module, the input \(\mathbf{X}\in\mathbb{R}^{B\times T\times d_{\text{hidden}}}\) is projected into query, key, and value tensors using three parameter matrices \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) for attention computation and generate \( \mathbf{X}_\text{Attn} \in \mathbb{R}^{B\times T\times d_{\text{hidden}}} \), which will be projected into \(\mathbf{W}^{\top}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\). Since \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v}\) operates on the same input, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{hidden}}\times d_{\text{hidden}}}\) for \( \mathbf{W}^{\top}_\mathrm{o} \) should be applied identically to the others' output channels:

\begin{equation}
\begin{aligned}
\widehat{\mathbf{W}}^{\top}_\mathrm{q} = \mathbf{W}^{\top}_\mathrm{q} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{k} = \mathbf{W}^{\top}_\mathrm{k} \mathbf{P}^{\top}_{\text{in}}, \\
\widehat{\mathbf{W}}^{\top}_\mathrm{v} = \mathbf{W}^{\top}_\mathrm{v} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{o} = \mathbf{P}_{\text{in}} \mathbf{W}^{\top}_\mathrm{o}.
\end{aligned}
\label{eq:3}
\end{equation}


% To maintain downstream consistency, the corresponding output projection matrix \(\mathbf{W}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) must absorb the inverse permutation on its input channels:
% $\mathbf{W}_o^{\prime} = \mathbf{W}_o \mathbf{P}_{\text{in}}^{\top}$.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{LaTeX/Figures/transformer_perm.pdf} 
\caption{An overview of channel permutation for Transformer layers. $\mathbf{W}_\mathrm{q}$, $\mathbf{W}_\mathrm{k}$, and $\mathbf{W}_\mathrm{v}$ need to learn their input channel permutation in an aggregated way and make corresponding adjustments in their output channel for $\mathbf{W}_\mathrm{o}$'s input channel permutation. $\mathbf{W}_\mathrm{gate}$ and $\mathbf{W}_\mathrm{up}$ are congruent.}
\label{fig:transformer_perm}
\vspace{-4mm}
\end{figure}


Similarly, the permutation of the input channel for \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \) requires implementation of the corresponding output channel permutation for the previous layer. The FFN submodule typically consists of two parallel expansion matrices \(\mathbf{W}^{\top}_{\mathrm{up}}, \mathbf{W}^{\top}_{\mathrm{gate}} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{ff}}}\) followed by a down-projection \(\mathbf{W}^{\top}_{\mathrm{down}} \in \mathbb{R}^{d_{\text{ff}} \times d_{\text{hidden}}}\). The two expansion paths operate on the same input and their outputs are combined multiplicatively. Therefore, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{ff}}\times d_{\text{ff}}}\) for \( \mathbf{W}^{\top}_\mathrm{down} \) should be applied identically to the others' output channels:


\begin{equation}
\resizebox{0.43\textwidth}{!}{$
\begin{aligned}
\widehat{\mathbf{W}}_{\mathrm{up}} =  \mathbf{W}^{\top}_{\mathrm{up}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{gate}} =  \mathbf{W}^{\top}_{\mathrm{gate}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{down}} =  \mathbf{P}_{\text{in}}\mathbf{W}^{\top}_{\mathrm{down}}.
\end{aligned}$}
\label{eq:4}
\end{equation}

\begin{figure*}[t]
\centering
\includegraphics[width=0.92\textwidth, height=0.32\textheight]{LaTeX/Figures/overview_new.pdf} 
\vspace{-0mm}
\caption{Overview of our learnable permutation framework. A permutation cost predictor generates cost matrices for each linear layer, which are converted into permutation matrices via a differentiable bipartite matching solver. The original weights are permuted accordingly and then sparsified using an N:M mask generator. During training, the pruned weights are inversely permuted and used for loss computation. The entire process supports end-to-end optimization while maintaining gradient flow through the binary permutation matrix generated by the differentiable solver.}
\label{fig:overview}
\vspace{-4mm}
\end{figure*}

These constraints highlight the key challenge: channel permutation in Transformers cannot be applied independently to each weight matrix, but must instead follow structured, group-consistent rules that preserve functional dependencies within each block. As such, we design our permutation system to operate jointly over grouped parameters, enforcing permutation sharing and inverse propagation where required. This ensures that permutation-aware sparsification maintains semantic alignment and preserves compatibility with structured weight compression.



\subsection{Learnable Channel Permutator}
\label{sec:perm}
To support semi-structured N:M sparsity constraint in Transformer models, we propose a learnable channel permutation framework that enables end-to-end optimization of permutation operators. It adaptively reorders input and output channels to align salient weights with fixed pruning patterns, improving weight retention within each group.

As shown in Fig.~\ref{fig:overview}, the framework consists of a permutation cost predictor, a differentiable bipartite matching solver, and a sparsity-aware training objective. The cost predictor produces layer-wise cost matrices, which are used to generate permutation matrices. These reorder the weights before pruning by an N:M mask generator. During training, pruned weights are inversely permuted for loss computation, preserving gradient flow through the pipeline.
Unlike heuristic approaches based on local importance or static ranking, our method learns permutation jointly across gradient-based end-to-end optimization. 
% To support structured pruning under the N:M sparsity constraint in Transformer-based architectures, we introduce a learnable channel permutation framework that enables end-to-end optimization of permutation operators. The core idea is to adaptively reorder the input and output channels of weight matrices such that the resulting structure is more compatible with fixed pruning patterns. This is especially critical in N:M sparsity, where preserving the most informative weights within each group requires aligning saliency patterns with the imposed structure.

% Our framework consists of three components: a permutation cost predictor, a differentiable bipartite matching solver, and a sparsity-aware training objective. Unlike prior heuristics that rely on local importance scores or static channel ranking, our method learns permutation jointly and differentiably across layers. By modeling the permutation process as a differentiable matching problem, we enable global coordination and gradient-based optimization. The cost predictor is trained with supervision from both final-task cross-entropy loss and intermediate layer-wise feature distillation, allowing the learned permutation to capture both global semantic alignment and structural sparsity compatibility.



\paragraph{Permutation Cost Predictor.}
\label{sec:cost}
The core of our method is a learnable permutation cost predictor, which produces a cost matrix to guide the reordering of channels or features. 
Given a weight matrix \(\mathbf{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}\) from a weight matrix, the goal is to construct a permutation matrix \(\mathbf{P} \in \{0,1\}^{d_{\text{in}} \times d_{\text{in}}}\) that rearranges the input channels such that the pruned model aligns more effectively with structured N:M sparsity constraints.

To enable differentiable learning of \(\mathbf{P}\), we introduce a real-valued cost matrix \(\mathbf{C} \in \mathbb{R}^{d_{\text{in}} \times d_{\text{in}}}\), where each element \(C_{i,j}\) reflects the cost of assigning the original input channel \(i\) to position \(j\). Intuitively, \(\mathbf{C}\) encodes the pairwise preference for spatial relocation, integrating both structured sparsity alignment and semantic preservation objectives.
We parameterize the cost matrix using  learnable parameters. For each input channel, we implement a \(d_{\text{in}} \times d_{\text{in}}\) learnable parameter as the cost predictor. 
The predictor outputs a normalized cost matrix, which quantifies the cost of swapping two input channels. We minimize the cumulative cost of each cost matrix with our proposed  bipartite matching solver. Our experimental results (Table~\ref{tab:vit_results}) demonstrate that the proposed permutation cost predictor achieves strong pruning performance despite its simple design, which is intentionally lightweight to minimize additional training overhead.

Furthermore, directly learning full permutation matrices for large-dimensional weight tensors in Transformer models is computationally expensive and often unnecessary. To improve scalability and reduce overhead, we adopt a group-wise permutation strategy, where the input channels of each layer are partitioned into non-overlapping groups size \(G\), and a separate permutation is learned within each group. This design not only reduces the number of parameters in the permutation predictor and solver, but also aligns naturally with hardware-efficient structured pruning, where pruning is applied in fixed-size blocks.

%we extract a feature vector \(f_i\) that summarizes the channel’s statistical or semantic properties, such as magnitude, variance, or learned embeddings. These features are first augmented with relative positional encodings to encode target indices \(j\), then passed through a  MLP layer \(h_\theta\) to produce the score:

%\begin{equation}
%    C_{i,j} = h_\theta\big(\text{concat}(f_i, \mathrm{PE}(j))\big),
%    \label{eq:5}
%\end{equation}
%where \(\mathrm{PE}(j)\) denotes the positional encoding of index \(j\). This formulation allows the predictor to model both channel-wise importance and positional compatibility jointly.
%The resulting cost matrix serves as the input to the differentiable matching solver.



%{\textcolor{blue}{Not clear for $C$. Is $C$ the input or output of the MLP? Does the MLP participate in the inference process of the original Transformer? What is the specific structure of the MLP?
%Also, how does $P$ affect $W$? Use a formula such as $W'=P*W$ or something to connect them.}

% \noident \textbf{Bipartite Matching Solver.}
% To obtain the optimal permutation matrix 
% $P^*$, we formulate the channel reordering problem as a bipartite matching task based on the cost matrix $C$. The objective is to solve:

% \begin{equation}
% {P^* = \arg\min_{P \in \mathcal{P}} \sum_{i=1}^{d_{\text{in}}} \sum_{j=1}^{d_{\text{in}}} P_{i,j} \cdot C_{i,j}
% \end{equation}
% where $\mathcal P$ denotes the set of valid permutation matrices (\textit{i.e.,} each row and column sums to 1). We use a differentiable matching solver (\textit{e.g.,} Gumbel-Sinkhorn [Mena et al.], SoftSort, or SparseSinkhorn) to allow gradient propagation through the discrete assignment process. The resulting soft permutation matrix is optionally binarized during inference to enable hardware-friendly structured sparsity.



\paragraph{Differentiable Bipartite Matching Solver.}
\label{sec:match}
To enable end-to-end optimization of the permutator, we design a differentiable bipartite matching solver that learns discrete permutation matrices in a gradient-friendly manner. As illustrated in Fig.~\ref{fig:diff_perm}, the module begins with a learned cost matrix and applies a Gumbel-Sinkhorn-based relaxation to approximate the optimal permutation in a differentiable form. During inference, it is converted into a discrete matrix using the Hungarian algorithm. In the following, we walk through each component of this solver, from group-wise matching to soft relaxation and final discretization.

Formally, given a predicted cost matrix \(\mathbf{C} \in \mathbb{R}^{N \times N}\) for a single group, where $N$ is size of a group of input weights, we frame channel permutation as a bipartite matching problem. The objective is to find a permutation matrix \(\mathbf{P} \in \mathcal{P}\), where \(\mathcal{P}\) denotes the set of \(N \times N\) permutation matrices, that minimizes the total matching cost:

\begin{equation}
    \min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle.
    \label{eq:6}
\end{equation}


However, this combinatorial optimization is non-differentiable and incompatible with gradient-based training. To enable end-to-end learning, we adopt a continuous relaxation by replacing \(\mathcal{P}\) with the Birkhoff polytope \(\mathcal{B}_N\), the convex hull of all permutation matrices:

\begin{equation}
    \mathcal{B}_N = \left\{ \mathbf{P} \in \mathbb{R}^{N \times N} \,\middle|\, \mathbf{P} \ge 0,\; \mathbf{P} \mathbf{1} = \mathbf{1},\; \mathbf{P}^{\top} \mathbf{1} = \mathbf{1} \right\}.
    \label{eq:7}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm.pdf} 
\caption{Learning a permutation with differentiable biparatite matching. A cost matrix $C$ is perturbed by independent Gumbel noise $g$ and converted to a kernel \(\exp\!\big(-(C+g)/\varepsilon\big)\). Sinkhorn iterations produce a soft doubly stochastic matrix \(P\) for training. At inference, Hungarian discretization yields a hard permutation that maximizes \(\sum_{i}\log P_{i,\Pi(i)}\). All steps before discretization are differentiable.}
\label{fig:diff_perm}
\vspace{-4mm}
\end{figure}


We then solve the entropy-regularized optimal transport problem:

\begin{equation}
\min_{\mathbf{P} \in \mathcal{B}_N} \langle \mathbf{C}, \mathbf{P} \rangle + \varepsilon \sum_{i,j} P_{ij} (\log P_{ij} - 1),
    \label{eq:8}
\end{equation}

which admits a solution of the form \(\mathbf{P} = \mathrm{Diag}(u)\, \mathbf{K} \, \mathrm{Diag}(v)\), where \(\mathbf{K} = \exp(-\mathbf{C} / \varepsilon)\). The scaling vectors \(u\) and \(v\) are computed via Sinkhorn iterations in the log domain:


\begin{equation}
\begin{aligned}
& \log u \leftarrow -\,\mathrm{logsumexp}(\log \mathbf{K} + \log v,\; \text{dim}=1),
\\
& \log v \leftarrow -\,\mathrm{logsumexp}(\log \mathbf{K}^{\top} + \log u,\; \text{dim}=1).
\end{aligned}
\label{eq:9}
\end{equation}

This iterative process enforces doubly stochastic constraints while maintaining numerical stability. We anneal the temperature \(\varepsilon_t\) over iterations, which progressively sharpens the soft assignment \(\mathbf{P}\) toward a discrete permutation while preserving differentiability. The resulting \(\mathbf{P}\) is applied blockwise to reorder channels, e.g., \(\mathbf{W}' = \mathbf{P} \mathbf{W}\), allowing gradients to flow through the solver back into the cost predictor and upstream network.

At inference, we convert \(\mathbf{P}\) into a discrete permutation by solving the original assignment problem:

\begin{equation}
    \Pi = \arg\min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle,
    \label{eq:10}
\end{equation}


using the Hungarian algorithm, which yields an exact one-to-one mapping in \(O(N^3)\) time per group. This produces a hardware-efficient permutation suitable for structured sparse deployment.

The solver’s time and space complexity scale as \(O(N^2 T)\) and \(O(N^2)\) per group, respectively, where \(T\) is the number of Sinkhorn iterations. Since the procedure is applied independently to each group, the overall cost grows linearly with the number of groups and quadratically with group size, consistent with our scalability results.

In addition to the Sinkhorn-based solver, our framework supports alternative differentiable relaxations, including Gumbel-Sinkhorn for stochastic exploration, SoftSort for rank-sensitive objectives, and SparseSinkhorn for promoting sharper sparsity in the doubly stochastic matrix.




\subsection{End-to-End Optimization Objectives}
\label{sec:loss}

To enable joint learning of channel permutation and structured pruning, we train the framework using a composite loss function that integrates both task-level supervision and intermediate feature alignment. This promotes not only the retention of end-task performance but also structural consistency within the model.

\paragraph{Task-Level Cross-Entropy Loss.}
We apply a standard cross-entropy loss to the output of the pruned model, allowing the permutation parameters to be optimized directly for task performance. Let \(f_{\text{perm+prune}}(x)\) denote the output of the model after applying learned permutation followed by N:M structured pruning. The task loss is defined as:



\begin{equation}
\mathcal{L}_{\text{task}} = \mathrm{CE}(f_{\text{perm+prune}}(x),\, y),
\label{eq:11}
\end{equation}


where \(\mathrm{CE}(\cdot)\) is the cross-entropy loss and \(y\) is the ground-truth label. This loss ensures that the permutation contributes to preserving the discriminative capacity of the network.

\paragraph{Layer-Wise Distillation Loss.}
To preserve internal feature semantics despite pruning and permutation, we incorporate a layer-wise distillation loss that aligns intermediate representations between the original and the permuted-pruned models. Let \(h_l^{\text{orig}}\) and \(h_l^{\text{perm+prune}}\) denote the output features of the \(l\)-th layer in the original and permuted-pruned models, respectively. The distillation loss is defined as:


\begin{equation}
\mathcal{L}_{\text{distill}} = \sum_{l=1}^{L}  \| h_l^{\text{orig}} - h_l^{\text{perm+prune}} \|_2^2,
\label{eq:12}
\end{equation}


where \(L\) is the number of pruned layers. This objective loss encourages the permutator to preserve task-relevant internal representations, improving compatibility with the original model behavior.

\paragraph{Combined Optimization Loss.}
The total loss is a weighted combination of task-level and distillation objectives:

\begin{equation}
    \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \alpha \, \mathcal{L}_{\text{distill}},
    \label{eq:13}
\end{equation}

where \(\alpha\) is a hyperparameter controlling the influence of intermediate feature alignment. This joint objective provides both global task supervision and local structural guidance for effective permutation learning.


%\subsection{Training and Evaluation Process}
\subsection{Training and Inference Details}

\paragraph{Training.}  
We begin by collecting input feature statistics for each layer of the pretrained Transformer. Specifically, we perform several hundred forward passes to accumulate running estimates of activation means, which are later used by the structured pruning method (Wanda) adopted in our framework. After this preprocessing stage, all Transformer weights are frozen, and only the parameters of the permutation cost predictor remain trainable.

To preserve structural consistency in attention layers, we impose a synchronized permutation constraint across coupled projection matrices, such as \(\mathbf{W}_q\), \(\mathbf{W}_k\), and \(\mathbf{W}_v\). These matrices share the same input representation, and applying inconsistent permutations would disrupt their joint computation. %Prior heuristic permutation methods often ignore this constraint, resulting in mismatched projections that undermine both model functionality and compatibility with hardware-efficient execution. 
By enforcing a shared permutation across structurally dependent components, our method ensures correctness and preserves the potential for real-world acceleration under structured sparsity.


\paragraph{Inference.}  
At inference time, the learned permutation cost predictor is frozen. For each group of channels, we can obtain the optimal permutation matrix via our bipartite matching solver. These permutations are applied to reorder the weights of each layer, followed by the application of N:M sparsity masks generated by the structured pruning method (Wanda). The resulting pruned model, with permuted and sparsified weights, is then used for standard Transformer inference.







==> sections/methods_v5.tex <==
\section{Methods}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{Figures/perm_isbetter.pdf} 
\caption{The channel permutation process enhances the friendliness of the 2:4 sparsification, making the overall saliency of the pruning metric more preserved.}
\label{fig:channel-perm}
\vspace{-4mm}
\end{figure}


We begin by introducing preliminaries on channel permutation in the context of optimizing structured N:M sparsity for Transformers. We then describe our proposed end-to-end learnable permutation framework, which consists of a learnable cost prediction module, a differentiable bipartite matching solver, and  optimization objectives. 
The unified framework facilitates end-to-end optimization of permutation operators for diverse transformer-based architectures, including vision, language, and vision-language models.



\subsection{Preliminaries}
\label{sec:preliminaries}

\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm_between_layers.pdf} 
\caption{Channel permutation for Linear layers. To guarantee output consistency, after the input channel of the $i$-th layer weight is permuted, the input activation of that layer should also be permuted accordingly, which can be realized by permuting the output channel of the previous ($i-1$)-th layer weight accordingly.}
\label{fig:perm_between_layers}
\vspace{-4mm}
\end{figure}

\paragraph{Optimize N:M Sparsity via Channel Permutation.} 
Channel permutation enhances the compatibility of weight tensors with structured sparsity patterns such as N:M sparsity. As shown in Figure~\ref{fig:channel-perm}, the weight layout often exhibits uneven saliency, with important weights clustered within certain groups. This skewed distribution lowers the chance of retaining key weights under fixed 2:4 sparsity, resulting in suboptimal pruning with reduced preserved saliency.

By permuting channels before pruning, saliency becomes more evenly distributed across groups. This increases the likelihood that each M-element group contains a mix of important and unimportant weights, allowing structured pruning to retain more informative elements. Channel permutation thus improves N:M pruning by aligning weight layout with sparsity constraints.

% To effectively apply channel permutation for structured sparsity, it is essential to consider how permutation interacts with the computational graph of the model. In practice, modern architectures consist of a variety of structural units, ranging from simple linear layers to highly interdependent Transformer blocks. We therefore analyze channel permutation in two representative settings: linear layers, where permutation can be propagated analytically between adjacent layers, and Transformer blocks, which require more careful coordination due to shared and coupled weight structures across multiple projections.


\paragraph{Channel Permutation for Linear Layers.} 
Applying a channel permutation to a linear layer's input dimension requires aligning the permuted weights with its input activation to preserve output consistency. Let \(\mathbf{W}_i^{\top} \in \mathbb{R}^{d_\text{in} \times d_\text{out}}\) be the weight matrix of the \(i\)-th linear layer, and let \(\mathbf{P}\in \{0,1\}^{d_\text{in} \times d_\text{in}}\) be a permutation matrix. Applying input channel permutation to the weight yields \(\widehat{\mathbf{W}}_i^{\top} = \mathbf{P} \mathbf{W}_i^{\top}\). To maintain correct computation, the corresponding activation \(\mathbf{A}_i \in \mathbb{R}^{d_\text{batch} \times d_\text{in}}\) must also be transformed as \(\widehat{\mathbf{A}}_i = \mathbf{A}_i \mathbf{P}^{\top}\), so that the output remains unchanged (\(\mathbf{P}^{\top} = \mathbf{P}^{-1}\)):

\begin{equation}
   \widehat{\mathbf{A}}_{i+1} = \widehat{\mathbf{A}}_i \widehat{\mathbf{W}}_i^{\top} = \mathbf{A}_i \mathbf{P}^{\top} \mathbf{P} \mathbf{W}_i^{\top} = \mathbf{A}_i \mathbf{W}_i^{\top} = \mathbf{A}_{i+1}, 
   \label{eq:1}
\end{equation}

% where the last equality holds since .

To avoid runtime activation permutation, we propagate the permutation backward to the output channels of the preceding \((i{-}1)\)-th layer: \(\widehat{\mathbf{W}}_{i-1} = \mathbf{W}_{i-1} \mathbf{P}^{\top}\), so that

\begin{equation}
    \widehat{\mathbf{A}}_i = \mathbf{A}_{i-1} \widehat{\mathbf{W}}_{i-1} = \mathbf{A}_{i-1} \mathbf{W}_{i-1} \mathbf{P}^{\top} = \mathbf{A}_i \mathbf{P}^{\top}.
    \label{eq:2}
\end{equation}

This transformation ensures functional equivalence without requiring explicit reordering of activations at runtime, as illustrated in Figure~\ref{fig:perm_between_layers}.


\paragraph{Channel Permutation for Transformer Layers.} 
Applying channel permutation in Transformer architectures presents unique challenges due to the complex structural coupling within multi-head self-attention (MHA) and feed-forward network (FFN) submodules. Unlike sequential linear layers, Transformer blocks involve parallel projections that share input representations and interdependent weight matrices, requiring permutation to be applied in a coordinated and structure-aware manner, as shown in Figure~\ref{fig:transformer_perm}.

In the MHA module, the input \(\mathbf{X}\in\mathbb{R}^{B\times T\times d_{\text{hidden}}}\) is projected into query, key, and value tensors using three parameter matrices \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) for attention computation and generate \( \mathbf{X}_\text{Attn} \in \mathbb{R}^{B\times T\times d_{\text{hidden}}} \), which will be projected into \(\mathbf{W}^{\top}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\). Since \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v}\) operates on the same input, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{hidden}}\times d_{\text{hidden}}}\) for \( \mathbf{W}^{\top}_\mathrm{o} \) should be applied identically to the others' output channels:

\begin{equation}
\begin{aligned}
\widehat{\mathbf{W}}^{\top}_\mathrm{q} = \mathbf{W}^{\top}_\mathrm{q} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{k} = \mathbf{W}^{\top}_\mathrm{k} \mathbf{P}^{\top}_{\text{in}}, \\
\widehat{\mathbf{W}}^{\top}_\mathrm{v} = \mathbf{W}^{\top}_\mathrm{v} \mathbf{P}^{\top}_{\text{in}}, \quad
\widehat{\mathbf{W}}^{\top}_\mathrm{o} = \mathbf{P}_{\text{in}} \mathbf{W}^{\top}_\mathrm{o}.
\end{aligned}
\label{eq:3}
\end{equation}


% To maintain downstream consistency, the corresponding output projection matrix \(\mathbf{W}_\mathrm{o} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{hidden}}}\) must absorb the inverse permutation on its input channels:
% $\mathbf{W}_o^{\prime} = \mathbf{W}_o \mathbf{P}_{\text{in}}^{\top}$.

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{LaTeX/Figures/transformer_perm.pdf} 
\caption{An overview of channel permutation for Transformer layers. $\mathbf{W}_\mathrm{q}$, $\mathbf{W}_\mathrm{k}$, and $\mathbf{W}_\mathrm{v}$ need to learn their input channel permutation in an aggregated way and make corresponding adjustments in their output channel for $\mathbf{W}_\mathrm{o}$'s input channel permutation. $\mathbf{W}_\mathrm{gate}$ and $\mathbf{W}_\mathrm{up}$ are congruent.}
\label{fig:transformer_perm}
\vspace{-4mm}
\end{figure}


Similarly, the permutation of the input channel for \(\mathbf{W}^{\top}_\mathrm{q}, \mathbf{W}^{\top}_\mathrm{k}, \mathbf{W}^{\top}_\mathrm{v} \) requires implementation of the corresponding output channel permutation for the previous layer. The FFN submodule typically consists of two parallel expansion matrices \(\mathbf{W}^{\top}_{\mathrm{up}}, \mathbf{W}^{\top}_{\mathrm{gate}} \in \mathbb{R}^{d_{\text{hidden}} \times d_{\text{ff}}}\) followed by a down-projection \(\mathbf{W}^{\top}_{\mathrm{down}} \in \mathbb{R}^{d_{\text{ff}} \times d_{\text{hidden}}}\). The two expansion paths operate on the same input and their outputs are combined multiplicatively. Therefore, the input channel permutation matrix \(\mathbf{P}_{\text{in}}\in\mathbb{R}^{d_{\text{ff}}\times d_{\text{ff}}}\) for \( \mathbf{W}^{\top}_\mathrm{down} \) should be applied identically to the others' output channels:


\begin{equation}
\resizebox{0.43\textwidth}{!}{$
\begin{aligned}
\widehat{\mathbf{W}}_{\mathrm{up}} =  \mathbf{W}^{\top}_{\mathrm{up}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{gate}} =  \mathbf{W}^{\top}_{\mathrm{gate}}\mathbf{P}^{\top}_{\text{in}},
\widehat{\mathbf{W}}_{\mathrm{down}} =  \mathbf{P}_{\text{in}}\mathbf{W}^{\top}_{\mathrm{down}}.
\end{aligned}$}
\label{eq:4}
\end{equation}

\begin{figure*}[t]
\centering
\includegraphics[width=0.92\textwidth, height=0.32\textheight]{LaTeX/Figures/overview_new.pdf} 
\vspace{-0mm}
\caption{Overview of our learnable permutation framework. A permutation cost predictor generates cost matrices for each linear layer, which are converted into permutation matrices via a differentiable bipartite matching solver. The original weights are permuted accordingly and then sparsified using an N:M mask generator. During training, the pruned weights are inversely permuted and used for loss computation. The entire process supports end-to-end optimization while maintaining gradient flow through the binary permutation matrix generated by the differentiable solver.}
\label{fig:overview}
\vspace{-4mm}
\end{figure*}

These constraints highlight the key challenge: channel permutation in Transformers cannot be applied independently to each weight matrix, but must instead follow structured, group-consistent rules that preserve functional dependencies within each block. As such, we design our permutation system to operate jointly over grouped parameters, enforcing permutation sharing and inverse propagation where required. This ensures that permutation-aware sparsification maintains semantic alignment and preserves compatibility with structured weight compression.



\subsection{Learnable Channel Permutator}
\label{sec:perm}
To support semi-structured N:M sparsity constraint in Transformer models, we propose a learnable channel permutation framework that enables end-to-end optimization of permutation operators. % It adaptively reorders input and output channels to align salient weights with fixed pruning patterns, improving weight retention within each group.
As shown in Fig.~\ref{fig:overview}, the framework consists of a permutation cost predictor, a differentiable bipartite matching solver, and an optimization training objective. The cost predictor produces layer-wise cost matrices, which are used to generate permutation matrices. These reorder the weights before pruning by an N:M mask generator (actually structured sparsity pruning method, we use Wanda in this paper). During training, pruned weights are inversely permuted for loss computation, preserving gradient flow through the pipeline.
Unlike heuristic approaches based on local importance or static ranking, our method learns permutation jointly across gradient-based end-to-end optimization. 
% To support structured pruning under the N:M sparsity constraint in Transformer-based architectures, we introduce a learnable channel permutation framework that enables end-to-end optimization of permutation operators. The core idea is to adaptively reorder the input and output channels of weight matrices such that the resulting structure is more compatible with fixed pruning patterns. This is especially critical in N:M sparsity, where preserving the most informative weights within each group requires aligning saliency patterns with the imposed structure.

% Our framework consists of three components: a permutation cost predictor, a differentiable bipartite matching solver, and a sparsity-aware training objective. Unlike prior heuristics that rely on local importance scores or static channel ranking, our method learns permutation jointly and differentiably across layers. By modeling the permutation process as a differentiable matching problem, we enable global coordination and gradient-based optimization. The cost predictor is trained with supervision from both final-task cross-entropy loss and intermediate layer-wise feature distillation, allowing the learned permutation to capture both global semantic alignment and structural sparsity compatibility.



\paragraph{Permutation Cost Predictor.}
\label{sec:cost}
The core of our method is a learnable permutation cost predictor, which produces a cost matrix to guide the reordering of channels or features. 
Given a weight matrix \(\mathbf{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}\) from a weight matrix, the goal is to construct a permutation matrix \(\mathbf{P} \in \{0,1\}^{d_{\text{in}} \times d_{\text{in}}}\) that rearranges the input channels such that the pruned model aligns more effectively with structured N:M sparsity constraints.

To enable differentiable learning of \(\mathbf{P}\), we introduce a real-valued cost matrix \(\mathbf{C} \in \mathbb{R}^{d_{\text{in}} \times d_{\text{in}}}\), where each element \(C_{i,j}\) reflects the cost of assigning the original input channel \(i\) to position \(j\). Intuitively, \(\mathbf{C}\) encodes the pairwise preference for spatial relocation, integrating both structured sparsity alignment and semantic preservation objectives.
We parameterize the cost matrix using  learnable parameters. For each input channel, we implement a \(d_{\text{in}} \times d_{\text{in}}\) learnable parameter as the cost predictor. 
The predictor outputs a normalized cost matrix, which quantifies the cost of swapping two input channels. We minimize the cumulative cost of each cost matrix with our proposed  bipartite matching solver. Our experimental results (Table~\ref{tab:vit_results}) demonstrate that the proposed permutation cost predictor achieves strong pruning performance despite its simple design, which is intentionally lightweight to minimize additional training overhead.

Furthermore, directly learning full permutation matrices for large-dimensional weight tensors in Transformer models is computationally expensive and often unnecessary. To improve scalability and reduce overhead, we adopt a group-wise permutation strategy, where the input channels of each layer are partitioned into non-overlapping groups size \(G\), and a separate permutation is learned within each group. %This design not only reduces the number of parameters in the permutation predictor and solver, but also aligns naturally with hardware-efficient structured pruning, where pruning is applied in fixed-size blocks.

%we extract a feature vector \(f_i\) that summarizes the channel’s statistical or semantic properties, such as magnitude, variance, or learned embeddings. These features are first augmented with relative positional encodings to encode target indices \(j\), then passed through a  MLP layer \(h_\theta\) to produce the score:

%\begin{equation}
%    C_{i,j} = h_\theta\big(\text{concat}(f_i, \mathrm{PE}(j))\big),
%    \label{eq:5}
%\end{equation}
%where \(\mathrm{PE}(j)\) denotes the positional encoding of index \(j\). This formulation allows the predictor to model both channel-wise importance and positional compatibility jointly.
%The resulting cost matrix serves as the input to the differentiable matching solver.



%{\textcolor{blue}{Not clear for $C$. Is $C$ the input or output of the MLP? Does the MLP participate in the inference process of the original Transformer? What is the specific structure of the MLP?
%Also, how does $P$ affect $W$? Use a formula such as $W'=P*W$ or something to connect them.}

% \noident \textbf{Bipartite Matching Solver.}
% To obtain the optimal permutation matrix 
% $P^*$, we formulate the channel reordering problem as a bipartite matching task based on the cost matrix $C$. The objective is to solve:

% \begin{equation}
% {P^* = \arg\min_{P \in \mathcal{P}} \sum_{i=1}^{d_{\text{in}}} \sum_{j=1}^{d_{\text{in}}} P_{i,j} \cdot C_{i,j}
% \end{equation}
% where $\mathcal P$ denotes the set of valid permutation matrices (\textit{i.e.,} each row and column sums to 1). We use a differentiable matching solver (\textit{e.g.,} Gumbel-Sinkhorn [Mena et al.], SoftSort, or SparseSinkhorn) to allow gradient propagation through the discrete assignment process. The resulting soft permutation matrix is optionally binarized during inference to enable hardware-friendly structured sparsity.



\paragraph{Differentiable Bipartite Matching Solver.}
\label{sec:match}
To enable end-to-end optimization of the permutator, we design a differentiable bipartite matching solver that learns discrete permutation matrices in a gradient-friendly manner. As illustrated in Fig.~\ref{fig:diff_perm}, the module begins with a learned cost matrix and applies a Gumbel-Sinkhorn-based relaxation to approximate the optimal permutation in a differentiable form. During inference, it is converted into a discrete matrix using the Hungarian algorithm. In the following, we walk through each component of this solver, from group-wise matching to soft relaxation and final discretization.

Formally, given a predicted cost matrix \(\mathbf{C} \in \mathbb{R}^{N \times N}\) for a weight group, where \(N\) is the number of input channels, we aim to find an optimal channel permutation. Each element \(\mathbf{C}_{i,j}\) represents the cost of assigning the \(i\)th original channel to the \(j\)th permuted position. We formulate this as a bipartite matching problem, where the goal is to find a permutation matrix \(\mathbf{P} \in \mathcal{P}\) that minimizes the total assignment cost:
\begin{equation}
    \min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle.
    \label{eq:6}
\end{equation}
where\(\langle \mathbf{C}, \mathbf{P} \rangle = \sum_{i,j} \mathbf{C}_{i,j} \mathbf{P}_{i,j}\),   \(\mathcal{P}\) denotes the set of all \(N \times N\) permutation matrices, where each row and column contains a single 1 and all other entries are 0.

However, solving this combinatorial optimization directly is non-differentiable for gradient-based training. To this end, we adopt a continuous relaxation by replacing \(\mathcal{P}\) with the Birkhoff polytope \(\mathcal{B}_N\), the convex hull of all permutation matrices~\cite{mena2018learning}.
This relaxation allows us to optimize over a continuous space of doubly stochastic matrices, defined as:
\begin{equation}
\mathcal{B}_N = \left\{ \mathbf{P} \in \mathbb{R}^{N \times N} \,\middle|\, \mathbf{P} \ge 0,\; \mathbf{P} \mathbf{1} = \mathbf{1},\; \mathbf{P}^{\top} \mathbf{1} = \mathbf{1} \right\}
\label{eq:7}
\end{equation}
where each row and column of \({P}\) sums to 1, making it a valid soft approximation of a permutation matrix.

\begin{algorithm}[t]
\caption{Differentiable Bipartite Matching Solver}
\label{alg:matching}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Cost matrix $\mathbf{C} \in \mathbb{R}^{N \times N}$, temperature $\varepsilon > 0$, number of iterations $T$
\STATE \textbf{Output:} Soft permutation matrix $\mathbf{P}$, discrete permutation matrix $\Pi$

\STATE $\mathbf{K} \gets \exp(-\mathbf{C} / \varepsilon)$
\STATE $\log \mathbf{K} \gets \log(\mathbf{K})$
\STATE Initialize $\log u \gets \mathbf{0},\quad \log v \gets \mathbf{0}$


\FOR{$t = 1$ to $T$}
    \STATE $\log u \gets -\,\mathrm{logsumexp}(\log \mathbf{K} + \log v,\; \text{dim}=1)$
    \STATE $\log v \gets -\,\mathrm{logsumexp}(\log \mathbf{K}^{\top} + \log u,\; \text{dim}=1)$
\ENDFOR
\STATE $u \gets \exp(\log u),\quad v \gets \exp(\log v)$
\STATE $\mathbf{P} \gets \mathrm{Diag}(u)\, \mathbf{K}\, \mathrm{Diag}(v)$


\STATE $\Pi \gets \arg\min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle$ \COMMENT{Solve using Hungarian algorithm}
\STATE $\Pi_{i,j} \in \{0, 1\}$ (discrete one-to-one permutation)

\STATE \textbf{return} $\mathbf{P}$, $\mathbf{\Pi}$
\end{algorithmic}
\end{algorithm}


\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{LaTeX/Figures/perm.pdf} 
\caption{Learning a permutation with differentiable biparatite matching. A cost matrix $C$ is perturbed by independent Gumbel noise $g$ and converted to a kernel \(\exp\!\big(-(C+g)/\varepsilon\big)\). Sinkhorn iterations produce a soft doubly stochastic matrix \(P\) for training. At inference, Hungarian discretization yields a hard permutation that maximizes \(\sum_{i}\log P_{i,\Pi(i)}\). All steps before discretization are differentiable.}
\label{fig:diff_perm}
\vspace{-4mm}
\end{figure}

To efficiently approximate the optimal soft permutation in $\mathcal{B}_N$, we cast the relaxed problem as an entropy-regularized optimal transport objective. It balances matching accuracy and smoothness, and can be solved efficiently via Sinkhorn iterations~\cite{cuturi2013sinkhorn, mena2018learning}:
\begin{equation}
\min_{\mathbf{P} \in \mathcal{B}N} \langle \mathbf{C}, \mathbf{P} \rangle + \varepsilon \sum{i,j} P_{ij} (\log P_{ij} - 1),
\label{eq:8}
\end{equation}
where the first term minimizes the matching cost, and the second introduces entropy to encourage smoother, more stable solutions, controlled by a constant temperature $\varepsilon$. This problem admits a closed-form solution  \(\mathbf{P} = \mathrm{Diag}(u)\, \mathbf{K} \, \mathrm{Diag}(v)\), where \(\mathbf{K} = \exp(-\mathbf{C} / \varepsilon)\), and \(u\), \(v\) are computed using Sinkhorn iterations in the log domain:
\begin{equation}
\begin{aligned}
\log u &\leftarrow -\log \sum \exp(\log \mathbf{K} + \log v), \\
\log v &\leftarrow -\log \sum \exp(\log \mathbf{K}^\top + \log u).
\end{aligned}
\label{eq:9}
\end{equation}
This iterative process ensures the solution remains doubly stochastic and differentiable. We gradually anneal the temperature $\varepsilon$ over training steps, encouraging the soft assignment to approach a discrete permutation. The resulting permutation is then applied blockwise to reorder channels (\(\mathbf{W}' = \mathbf{P} \mathbf{W}\)), allowing gradients to flow through the solver back into the cost predictor and upstream network.

At inference time, we convert the soft assignment \(\mathbf{P}\) into a discrete permutation $\Pi$ by solving the original assignment problem:
\begin{equation}
\Pi = \arg\min_{\mathbf{P} \in \mathcal{P}} \langle \mathbf{C}, \mathbf{P} \rangle,
\label{eq:10}
\end{equation}
using the Hungarian algorithm~\cite{kuhn1955hungarian}, which guarantees a one-to-one binary mapping for each permutation matrix. 
In addition to the Sinkhorn-based solver, our framework supports alternative differentiable relaxations, including Gumbel-Sinkhorn for stochastic exploration, SoftSort for rank-sensitive objectives, and SparseSinkhorn for promoting sharper sparsity in the doubly stochastic matrix.




\subsection{End-to-End Optimization Objectives}
\label{sec:loss}

To enable joint learning of channel permutation and structured pruning, we train the framework using a composite loss function that integrates both task-level supervision and intermediate feature alignment. This promotes not only the retention of end-task performance but also structural consistency within the model.

\paragraph{Task-Level Cross-Entropy Loss.}
We apply a standard cross-entropy loss to the output of the pruned model, allowing the permutation parameters to be optimized directly for task performance. Let \(f_{\text{perm+prune}}(x)\) denote the output of the model after applying learned permutation followed by N:M structured pruning. The task loss is defined as:



\begin{equation}
\mathcal{L}_{\text{task}} = \mathrm{CE}(f_{\text{perm+prune}}(x),\, y),
\label{eq:11}
\end{equation}


where \(\mathrm{CE}(\cdot)\) is the cross-entropy loss and \(y\) is the ground-truth label. This loss ensures that the permutation contributes to preserving the discriminative capacity of the network.

\paragraph{Layer-Wise Distillation Loss.}
To preserve internal feature semantics despite pruning and permutation, we incorporate a layer-wise distillation loss that aligns intermediate representations between the original and the permuted-pruned models. Let \(h_l^{\text{orig}}\) and \(h_l^{\text{perm+prune}}\) denote the output features of the \(l\)-th layer in the original and permuted-pruned models, respectively. The distillation loss is defined as:


\begin{equation}
\mathcal{L}_{\text{distill}} = \sum_{l=1}^{L}  \| h_l^{\text{orig}} - h_l^{\text{perm+prune}} \|_2^2,
\label{eq:12}
\end{equation}


where \(L\) is the number of pruned layers. This objective loss encourages the permutator to preserve task-relevant internal representations, improving compatibility with the original model behavior.

\paragraph{Combined Optimization Loss.}
The total loss is a weighted combination of task-level and distillation objectives:

\begin{equation}
    \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{task}} + \alpha \, \mathcal{L}_{\text{distill}},
    \label{eq:13}
\end{equation}

where \(\alpha\) is a hyperparameter controlling the influence of intermediate feature alignment. This joint objective provides both global task supervision and local structural guidance for effective permutation learning.


%\subsection{Training and Evaluation Process}
\subsection{Training and Inference Details}

\paragraph{Training.}  
We begin by collecting input feature statistics for each layer of the pretrained Transformer. Specifically, we perform several hundred forward passes to accumulate running estimates of activation means, which are later used by the structured pruning method (Wanda) adopted in our framework. After this preprocessing stage, all Transformer weights are frozen, and only the parameters of the permutation cost predictor remain trainable.

To preserve structural consistency in attention layers, we impose a synchronized permutation constraint across coupled projection matrices, such as \(\mathbf{W}_q\), \(\mathbf{W}_k\), and \(\mathbf{W}_v\). These matrices share the same input representation, and applying inconsistent permutations would disrupt their joint computation. %Prior heuristic permutation methods often ignore this constraint, resulting in mismatched projections that undermine both model functionality and compatibility with hardware-efficient execution. 
By enforcing a shared permutation across structurally dependent components, our method ensures correctness and preserves the potential for real-world acceleration under structured sparsity.


\paragraph{Inference.}  
At inference time, the learned permutation cost predictor is frozen. For each group of channels, we can obtain the optimal permutation matrix via our bipartite matching solver. These permutations are applied to reorder the weights of each layer, followed by the application of N:M sparsity masks generated by the structured pruning method (Wanda). The resulting pruned model, with permuted and sparsified weights, is then used for standard Transformer inference.







==> sections/related_work.tex <==
\section{Related Work}
\subsection{Model Pruning}
Model pruning aims to produce a compressed variant of a pre-trained model by reducing storage requirements, memory bandwidth, and computational cost. Recent pruning methods can be broadly categorized into three main types. 
Firstly, \textbf{unstructured pruning} removes individual weight parameters, allowing fine-grained control over sparsity. However, the resulting irregular memory access often restricts practical acceleration to a small subset of devices or requires extreme sparsity, which can degrade model accuracy~\cite{han2015deep_compression, han2015learning}. 
Secondly, \textbf{(pure-) structured pruning} removes entire filters, channels, or layers, resulting in coarse-grained but hardware-friendly model compression. However, this often leads to significant performance degradation and typically requires retraining to restore accuracy~\cite{ma2023llmpruner, xia2023sheared, he2017channel}.
Finally, \textbf{(semi-) structured pruning}, also known as N:M sparsity, offers a trade-off by enforcing a fixed number of nonzero weights within small groups. It preserves much of the accuracy of unstructured pruning while enabling regular memory layouts that modern accelerators can efficiently exploit for high throughput~\cite{pool2021accelerating, pool2021channel, frantar2023sparsegpt}.



\subsection{N:M Sparsity}
The N:M sparsity pattern constrains each block of M weights to contain at most N nonzero elements, providing a balance between high compression ratios and efficient execution on specialized hardwares~\cite{pool2021accelerating, pool2021channel, fang2024maskllm}. 
Early approaches applied static N:M masks after training. In contrast, recent work integrates mask generation into the optimization process by employing continuous relaxations of the discrete sparsity pattern and using gradient-based updates to jointly learn weights and mask scores~\cite{zhou2021learning,lu2023step}. Techniques such as sparse-refined straight-through estimators further encourage important weights to remain nonzero while strictly enforcing the N:M constraint~\cite{bengio2013estimating,han2015learning}.
% Scaling these approaches to multi‑billion‑parameter language models remains challenging due to the sheer number of mask variables and the desire to avoid costly fine‑tuning.


\subsection{Matrix Permutation}
Matrix permutation approaches aim to redistribute salient and non-salient weights more evenly across subblocks. This reordering facilitates better alignment with structured sparsity patterns such as N:M sparsity, ultimately improving pruning compatibility and preserving model performance. 
\sout{By learning optimal permutations or using heuristic strategies, these methods enhance block-wise saliency balance without changing the global sparsity level~\cite{pool2021channel,zhang2022learning}. Some advanced frameworks further integrate permutation learning with mask optimization to jointly refine both the sparsity pattern and model accuracy~\cite{shekhar2023end}.}
{\color{red} {Please only cite greedy or heuristic method here!!!!!!!!}}

\vskip 1em
\noindent In this work, we tackle the large search space of channel permutations by introducing a learnable permutation mechanism for GPT-scale Transformers. Our method enables effective channel reordering that improves model accuracy under N:M sparsity constraints.
